RKHS Representation of Algebraic Convolutional Filters with Integral Operators

Integral operators play a central role in signal processing, underpinning classical convolution, and filtering on continuous network models such as graphons. While these operators are traditionally analyzed through spectral decompositions, their connection to reproducing kernel Hilbert spaces (RKHS) has not been systematically explored within the algebraic signal processing framework. In this paper, we develop a comprehensive theory showing that the range of integral operators naturally induces RKHS convolutional signal models whose reproducing kernels are determined by a box product of the operator symbols. We characterize the algebraic and spectral properties of these induced RKHS and show that polynomial filtering with integral operators corresponds to iterated box products, giving rise to a unital kernel algebra. This perspective yields pointwise RKHS representations of filters via the reproducing property, providing an alternative to operator-based implementations. Our results establish precise connections between eigendecompositions and RKHS representations in graphon signal processing, extend naturally to directed graphons, and enable novel spatial--spectral localization results. Furthermore, we show that when the spectral domain is a subset of the original domain of the signals, optimal filters for regularized learning problems admit finite-dimensional RKHS representations, providing a principled foundation for learnable filters in integral-operator-based neural architectures.

==> figures/algnn_one_layer.tex <==
%!TEX root = ../../lecture_\ell2_compile_handout/lecture_\ell2_handout.tex

%-- Viridis Color Palette
\definecolor{my_cp5_col1}{RGB}{253, 231, 37}
\definecolor{my_cp5_col2}{RGB}{94, 201, 98}
\definecolor{my_cp5_col3}{RGB}{33, 145, 140}
\definecolor{my_cp5_col4}{RGB}{59, 82, 139}
\definecolor{my_cp5_col5}{RGB}{68, 1, 84}

\def \myfactor {0.8}
\def \unit  {\myfactor cm}

% Definition of a block for block diagrams
\tikzstyle{block} = [ rectangle,
                      minimum width = \unit,
                      minimum height = \unit,
                      fill = blue!15,
                      draw = black,
                      text = black]

% Control the color and size of filter blocks
\tikzstyle{filter} = [block,
                      minimum width  = 3.0*\unit,
                      minimum height = 1.3*\unit,
                      fill=my_cp_col5]

% Control the color and size of nonlinearity blocks
\tikzstyle{nonlinearity} = [ filter,
                             minimum width  = 2.5*\unit,
                             fill = my_cp_col4]

% Control separation between blocks
\def \deltainput     {( 0.0,-1.7)}
\def \deltaoutput    {( 0.0,-1.2)}
\def \deltalayer     {3.2}
\def \deltaconnector {1.45}
\def \deltasigma     {( 3.8, 0.0)}
\def \deltasigmab    {( 3.5, 0.0)}

% The text that is displayed inside of filter blocks
\def \one {$\textcolor{white}{\displaystyle{\boldsymbol{y}^{\ell}_m = \sum_{n=1}^{N_{\ell-1}}h_{n,m}^{\ell} \ast\boldsymbol{x}_n^{\ell-1}}}$}

% The text that is displayed inside of nonlinearity blocks
\def \sigmaone   {$\textcolor{white}{\displaystyle{\boldsymbol{x}_{\ell} = {\eta_{\ell}} \Big[\, \boldsymbol{y}_{\ell} \, \Big]}}$}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% BEGIN FIGURE CODE %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
{\fontsize{8}{8}\selectfont\begin{tikzpicture}[scale = \myfactor]

  \pgfdeclarelayer{bg}     % declare background layer
  \pgfsetlayers{bg,main}   % set the order of the layers (main is the standard layer)

  % Draw input to GNN
  \node (input) [rectangle, minimum width = 0.1*\unit] {$\boldsymbol{x}_{\ell\text{-}1}=\left(x_1^{\ell\text{-}1}, \hdots, x_{N_{\ell\text{-}1}}^{\ell\text{-}1}\right)$};
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  % Layer 1 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  % Draw Layer 1 Filter block and Feature block
  \path (input.east)      ++ \deltainput node [filter]       (L1 Filter1) {\one};
  \path (L1 Filter1) ++ \deltasigma node [nonlinearity] (L1 F1)      {\sigmaone};
  % Draw connectors for Layer 1
  \path[draw, -stealth] (L1 Filter1.east) -- node [above] {$\boldsymbol{y}_\ell$} (L1 F1.west);

  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  % Connections across layers %%%%%%%%%%%%%%%%%%%%%%
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  % From input to layer 1
  \path[draw, -stealth] (input.east) -- (L1 Filter1.north);
  % From layer 1 to layer 2
  \path (L1 F1.south) ++ (0,-\deltaconnector) node [] (aux1) {};
  \path[draw, -stealth] (L1 F1.south) -- (aux1.north) node [right] {$\boldsymbol{x}_\ell=\left(x_1^{\ell}, \hdots, x_{N_{\ell}}^{\ell}\right)$} ;

  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  % Light shades to signify layer groups   %%%%%%%%%
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  \begin{pgfonlayer}{bg}
      % Shading for Layer 1
      \path (L1 Filter1.west |- L1 F1.south) ++ (-0.3,-0.5)
           node [filter, anchor = south west,
                 fill = black!5,
minimum width  = 7.5*\unit,
minimum height = 2.0*\unit,
]
        (layer)
        {};
       \path (layer.south west) ++ (0.0,0.0) node [above right] {Layer $\ell$};
   \end{pgfonlayer}

\end{tikzpicture}}


==> figures/asp_diagrams/fig2_tikz_source.tex <==
%!TEX root = ../../compiler_paper.tex




%%%%%%%%%%%%%%%%%%%%%%% Colors %%%%%%%%%%%%%%%%%%%%



%-- Viridis Color Palette
%% ----- Viridis color palette -----
\definecolor{my_cp_col1}{RGB}{253, 231, 37}
\definecolor{my_cp_col2}{RGB}{180, 222,44}
\definecolor{my_cp_col3}{RGB}{94, 201, 98}
\definecolor{my_cp_col4}{RGB}{33, 145, 140}
\definecolor{my_cp_col5}{RGB}{59, 82, 139}
\definecolor{my_cp_col6}{RGB}{68, 1, 84}





\usetikzlibrary{positioning,decorations.pathreplacing,shapes}
%\usepackage[english]{babel}
%\usepackage{microtype}
%\usepackage[hmargin=1.5cm,vmargin=1cm]{geometry}
%\usepackage{amsmath}
%\DeclareMathOperator{\p}{p}
%\newcommand*{\cancer}{\text{cancer}}
%\newcommand*{\testp}{\text{test}+}



%%%%%%%%%%%%%%%%%%%%%%%%%%% Settings of Blocks and picture %%%%%%%%%%%%%%%%%%%

\def \scale {1.3}
\def \unit  { \scale cm}
\def \layerinterdist {4}


% Block styles
\tikzstyle{set} = [rectangle,color=black,
                    rounded corners = 0.2*\unit,
                    fill=black,
                    inner sep=0pt,
                    draw,
                    anchor = center,
                    line width=0.1mm]
                                      
\tikzstyle{vectorspace} = [set, 
                             fill=my_cp_col5,
                             minimum width  = 2.5*\unit,
                             minimum height = 1.5451*\unit]
                             
\tikzstyle{endomorphisms} = [vectorspace,
                              fill=my_cp_col4]
                                
\tikzstyle{algebra} = [endomorphisms,
                        fill=my_cp_col2,
                         minimum width  = 2.5*\unit,
                        minimum height = 1.5451*\unit]

\tikzstyle{rec_box} = [endomorphisms,
                         rounded corners = 0*\unit,
                        fill=my_cp_col2,
                         minimum width  = 2.5*\unit,
                        minimum height = 1.5451*\unit]



\tikzstyle{dot} = [circle,
                    minimum width  = 0.12*\unit,
                    fill=black,
                    color=black,
                    inner sep=0pt,
                    draw,
                    anchor = center ]





{\fontsize{8}{8}\selectfont


\begin{tikzpicture}[rounded corners,ultra thick]


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%% Vector space M  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

   \path (0,0) node [vectorspace, fill opacity=1] (M0) {};
   \path (M0.south) ++ (0, 0.2) node [above, color=my_cp_col2] {$\mathcal{H}$};
   
   % Element of the vector space
   \path (M0) ++ (-1,0.2) node [dot,color=my_cp_col2] (x) {};
   \path (x.south)++(0,-0.1) node [below, color=my_cp_col2] {$\boldsymbol{x}$}; 
   
   % Element filtered in the vector space
   \path (M0) ++ (1,0.2) node [dot,color=my_cp_col2] (ex) {};
   \path (ex.south) node [below, color=my_cp_col2] {$\rho(\boldsymbol{a})\boldsymbol{x}$};      
              

% Comment about where the signals living in H
 \path (M0.south) ++ (0,0) node [] (Htext) {};
 \path (Htext.south) node [below, color=my_cp_col6,align=center] {Vector Space
   (Signals)}; 







%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%% Endomorphisms   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

   \path (M0.north) ++ (0, 1) 
         node [endomorphisms, anchor=south, fill opacity=1] (End0) {};
   \path (End0.north) ++ (0.0, -0.2) node [below, color=my_cp_col6] {$\mathcal{B}\left(\mathcal{H}\right)$}; 
   

   % Adding an endomorphism element 
   \path (End0.south) ++ (0.0, 0.6) node [dot,color=my_cp_col6] (e) {};      
   %\path (e) node [right] {$\rho(\boldsymbol{a})$};    
   \path (e.center) ++ (0.5,0.25) node [color=my_cp_col6] {$\rho(\boldsymbol{a})$}; 
   
   % Arrow going from x to Ex
   \path (e)+(-1,0.77) coordinate (c1);
   \path (e)+(1,0.77) coordinate (c2);   
   \path [draw, -stealth, line width=0.8,color=my_cp_col3] (x) .. controls (c1) and (c2) .. (ex);   

  

   
   
   
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%% Algebra %%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

   \path (End0.north west) ++ (-1, 0) 
         node [algebra, anchor = north east, fill opacity=1] (A) {};   
   \path (A.north) ++ (0,-0.2) node [below,color=my_cp_col6] {$\mathcal{A}$};
   \path (A.center) ++ (-0.25,0) node [below,color=my_cp_col6] {$\boldsymbol{a}$};  
   %\path (A.south) ++ (0,0.75) node [below,color=black, align=center] {};  
    
%  \path (subset2.south) ++ (0, 0.2) node [above, color=black] {$\mathcal{C}$};
    
    % Element in the Algebra
    \path (A.south) ++ (0.0, 0.6) node [dot,color=my_cp_col6] (a1) {}; 
        
   % Arrow indicating \rho going from A to End(M)  
   \path (A.north) + (1,-0.1) coordinate (c1);
   \path (End0.north) + (-1,-0.1) coordinate (c2);   
   \path [draw, -stealth,line width = 1,color=my_cp_col5,  opacity=1] (a1) .. controls (c1) and (c2) .. (e) node[midway,above left,rotate=0,color=black,opacity=1] {$\rho$};
   
   
% Comment about where the signals living in H
 \path (A.south) ++ (0,0) node [] (Atext) {};
 \path (Atext.south) node [below, color=my_cp_col6,align=center] {Algebra
   (Filters)}; 


   
   




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%  C O M M E N T S   A N D   T E X T   %%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%   
   
\path (A.south) ++ (0, -1) node [rec_box, anchor=north, fill opacity=0.2,color=my_cp_col1] (rectext) {};
   
% Comment about where the signals living in H
 \path (A.south) ++ (0,-0.9) node [] (Atext) {};
 \path (Atext.south) node [below, color=my_cp_col3,align=center] { $\ccalA\Rightarrow$ \textbf{Fundamental Laws}  \\
   \textbf{of convolution}};            
          
 % Comment about where the signals living in H
 \path (A.south) ++ (0,-1.8) node [] (Htext) {};
 \path (Htext.south) node [below, color=my_cp_col5] {$\ccalH\Rightarrow$ \textbf{Information (data)} };       
 
 
  % Comment about where the signals living in H
 \path (A.south) ++ (0,-2.4) node [] (Endtext) {};
 \path (Endtext.south) node [below, color=my_cp_col4] {$\rho\Rightarrow$ \textbf{Implements filters}};    

\end{tikzpicture}
}







==> figures/fig_15_tikz_source.tex <==
%!TEX root = ../compiler_paper.tex





%%-----------------------------------------------------------------
%%---------------  C O L O R S -------------------------------
%%-----------------------------------------------------------------

%**********  V I R I D I S   C. P a l e t t e   ***********
\definecolor{my_cp_col1}{RGB}{253, 231, 37}
\definecolor{my_cp_col2}{RGB}{180, 222,44}
\definecolor{my_cp_col3}{RGB}{94, 201, 98}
\definecolor{my_cp_col4}{RGB}{33, 145, 140}
\definecolor{my_cp_col5}{RGB}{59, 82, 139}
\definecolor{my_cp_col6}{RGB}{68, 1, 84}


%**********  Secondary Viridis Color Palette  (More pastel like)
\definecolor{my_cp2_col1}{RGB}{255,255,217}
\definecolor{my_cp2_col2}{RGB}{237,248,177}
\definecolor{my_cp2_col3}{RGB}{199,233,180}
\definecolor{my_cp2_col4}{RGB}{127,205,187}
\definecolor{my_cp2_col5}{RGB}{65,182,196}
\definecolor{my_cp2_col6}{RGB}{29,145,192}
\definecolor{my_cp2_col7}{RGB}{34,94,168}
\definecolor{my_cp2_col8}{RGB}{37,52,148}
\definecolor{my_cp2_col9}{RGB}{8,29,88}






%---------------------------------------------------------------------
%------  F I X   V A L U E S   A N D   S C A L E  ----------
%---------------------------------------------------------------------

%*******  S C A L E   A N D   U N I T  *******
\def \scale{2}
\def \unit {\scale cm}

%******  Ext  I M A G E S   S C A L E   ******
\def \imgscale{0.055}

%*****  H E I G H T  -  W I D T H - GoldenRatio   ******
\def\mywidth{4.5}
\def\myheight{\mywidth/1.618}

\def\stepx{0.9*\unit}
\def\stepy{0.9*\unit}

\def\mylinewidth{3}



%%-----------------------------------------------------------------
%%------------ B A S I C   F O R M S  ----------------------
%%-----------------------------------------------------------------

%*****  R E C T A N G U L A R   R E G I O N    *****

\tikzstyle{set} = [rectangle,color=black,
                    rounded corners = 0*\unit,
                    fill=black,
                    inner sep=0pt,
                    draw,
                    anchor = center,
                    line width=0.1mm]

\tikzstyle{rec_region} = [set,
                             fill=my_cp2_col3,
                             minimum width  = \mywidth*\unit,
                             minimum height = \myheight*\unit]


\tikzstyle{dot} = [circle,
                    minimum width  = 0.12*\unit,
                    fill=black,
                    color=black,
                    inner sep=0pt,
                    draw,
                    anchor = center ]










%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%   T I K Z   F I G U R E   B E G I N S   %%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

 \begin{tikzpicture}[myn/.style={circle,  thin, draw, inner sep=0.15cm, outer sep=2pt, ball color=my_cp4_col3}]




%%---------------------------------------------------------------------------
%%------------------  F O O T B A L L   F I E L D   ------------------
%%---------------------------------------------------------------------------

\path (0,0) node [rec_region, fill opacity=1, anchor=south west] (R) {};




%%---------------------------------------------------------------------------
%%----------  L I N E   D I V I D I N G   F I E L D   ----------------
%%---------------------------------------------------------------------------

% Vertical lines
\path (0,0)++(\mywidth,0)  coordinate (p1);
\path (0,0)++(\mywidth,\myheight*\unit) coordinate (p2);
\draw[my_cp2_col8, line width=\mylinewidth, opacity=0.7] (p1) -- (p2) ;





%%----------------------------------------------------------------------------
%%---------- K N O W N  P O S I T I O N S   D R O N  ----------
%%----------------------------------------------------------------------------

%***** Going up from the starting point

% Dron
\node[inner sep=0pt] (drone1a) at (0.5*\stepx,0.3*\stepy)
{\includegraphics[width=\imgscale\textwidth]{./figures/external_images/Img_2_opac}};
\path (drone1a)++(0.3*\stepx,0)  coordinate (p1);
\node[right, opacity=0.6] (x0) at (p1)  {$f(v_{0})$};

% Dron
\node[inner sep=0pt] (drone1a) at (0.5*\stepx,1*\stepy)
{\includegraphics[width=\imgscale\textwidth]{./figures/external_images/Img_2_opac}};

% Dron
\node[inner sep=0pt] (drone1a) at (0.5*\stepx,1.7*\stepy)
{\includegraphics[width=\imgscale\textwidth]{./figures/external_images/Img_2_opac}};
\path (drone1a)++(0.3*\stepx,0)  coordinate (p1);
\node[right, opacity=0.6] (x0) at (p1)  {$f(v_{2})$};

% Dron
\node[inner sep=0pt] (drone1a) at (0.5*\stepx,2.4*\stepy)
{\includegraphics[width=\imgscale\textwidth]{./figures/external_images/Img_2_opac}};



%***** Turning to the right *****

% Dron
\node[inner sep=0pt] (drone1a) at (1.1*\stepx,2.8*\stepy)
{\includegraphics[width=\imgscale\textwidth]{./figures/external_images/Img_2_opac}};
\path (drone1a)++(0*\stepx,-0.3*\stepy)  coordinate (p1);
\node[below, opacity=0.6] (x0) at (p1)  {$f(v_{4})$};

% Dron
\node[inner sep=0pt] (drone1a) at (2*\stepx,2.7*\stepy)
{\includegraphics[width=\imgscale\textwidth]{./figures/external_images/Img_2_opac}};


%***** Turning down *****

% Dron
\node[inner sep=0pt] (drone1a) at (2*\stepx,2*\stepy)
{\includegraphics[width=\imgscale\textwidth]{./figures/external_images/Img_2_opac}};

% Dron
\node[inner sep=0pt] (drone1a) at (2*\stepx,1.3*\stepy)
{\includegraphics[width=\imgscale\textwidth]{./figures/external_images/Img_2_opac}};

%% Dron
%\node[inner sep=0pt] (drone1a) at (2*\stepx,0.4*\stepy)
%{\includegraphics[width=\imgscale\textwidth]{./external_images/Img_2_opac}};

% Dron
\node[inner sep=0pt] (drone1a) at (2*\stepx,0.5*\stepy)
{\includegraphics[width=\imgscale\textwidth]{./figures/external_images/Img_2}};
\path (drone1a)++(-0.3*\stepx,0)  coordinate (p1);
\node[left, opacity=1] (x0) at (p1)  {$f(v_{8})$};




%%----------------------------------------------------------------------------
%%------ U N K N O W N  P O S I T I O N S   D R O N  --------
%%----------------------------------------------------------------------------

%***** Turning right and up*****

% Unknown point
\path (3*\stepx,0.5*\stepy)  node [dot, color=my_cp_col5, opacity=1] (a1) {};
\path (a1)++(0.3*\stepx,0)  coordinate (p1);
\node[right, opacity=0.6] (x0) at (p1)  {$r(v_{9})$};

% Unknown point
%\path (3*\stepx,1*\stepy)  node [dot, color=my_cp_col5, opacity=1] (a1) {};

% Unknown point
\path (3*\stepx,1.6*\stepy)  node [dot, color=my_cp_col5, opacity=1] (a1) {};


% Unknown point
\path (3*\stepx,2*\stepy)  node [dot, color=my_cp_col5, opacity=1] (a1) {};
\path (a1)++(0.3*\stepx,0)  coordinate (p1);
\node[right, opacity=0.6] (x0) at (p1)  {$r(v_{11})$};

% Unknown point
\path (3*\stepx,2.7*\stepy)  node [dot, color=my_cp_col5, opacity=1] (a1) {};


%*********  Turning right  ********

% Unknown point
%\path (3.5*\stepx,2.7*\stepy)  node [dot, color=my_cp_col5, opacity=1] (a1) {};

% Unknown point
\path (4*\stepx,2.7*\stepy)  node [dot, color=my_cp_col5, opacity=1] (a1) {};

% Unknown point
\path (4.6*\stepx,2.7*\stepy)  node [dot, color=my_cp_col5, opacity=1] (a1) {};


%*********  Turning  down  ********

% Unknown point
\path (4.6*\stepx,2.2*\stepy)  node [dot, color=my_cp_col5, opacity=1] (a1) {};

% Unknown point
%\path (4.6*\stepx,1.7*\stepy)  node [dot, color=my_cp_col5, opacity=1] (a1) {};

% Unknown point
%\path (4.6*\stepx,1.7*\stepy)  node [dot, color=my_cp_col5, opacity=1] (a1) {};

% Unknown point
\path (4.6*\stepx,1.1*\stepy)  node [dot, color=my_cp_col5, opacity=1] (a1) {};
\path (a1)++(-0.3*\stepx,0)  coordinate (p1);
\node[left, opacity=0.6] (x0) at (p1)  {$r(v_{16})$};

% Unknown point
\path (4.6*\stepx,0.4*\stepy)  node [dot, color=my_cp_col5, opacity=1] (a1) {};





%%----------------------------------------------------------------------------
%%-----------------------    A R R O W S  ------------------------------
%%----------------------------------------------------------------------------

%****** Going up arrow from initial point
\path (0,0)++(0.8*\stepx,0.2*\stepy)  coordinate (p1);
\path (0,0)++(0.8*\stepx,1.1*\stepy) coordinate (p2);
\draw[-stealth,my_cp_col5, line width=\mylinewidth, opacity=0.9] (p1) -- (p2) ;

%****** Going up - right - down  ********
\path (0,0)++(0.8*\stepx,1.5*\stepy)  coordinate (p1);
\path (0,0)++(0.8*\stepx,2.5*\stepy) coordinate (p2);
\path (0,0)++(1.5*\stepx,2.5*\stepy) coordinate (p3);
\draw[-stealth,my_cp_col5, line width=\mylinewidth, opacity=0.9,rounded corners = 0.2*\unit] (p1) -- (p2) -- (p3) ;

%****** Going up - down  ********
\path (0,0)++(1.7*\stepx,2.4*\stepy)  coordinate (p1);
\path (0,0)++(1.7*\stepx,1.1*\stepy) coordinate (p2);
\draw[-stealth,my_cp_col5, line width=\mylinewidth, opacity=0.9] (p1) -- (p2) ;

%****** Turning to the right  ********
\path (0,0)++(1.7*\stepx,0.8*\stepy)  coordinate (p1);
\path (0,0)++(1.7*\stepx,0.2*\stepy) coordinate (p2);
\path (0,0)++(3.3*\stepx,0.2*\stepy) coordinate (p3);
\path (0,0)++(3.3*\stepx,0.8*\stepy) coordinate (p4);
\draw[-stealth,my_cp_col5, line width=\mylinewidth, opacity=0.9,rounded corners = 0.2*\unit] (p1) -- (p2) -- (p3) -- (p4) ;

%****** Going up  ********
\path (0,0)++(3.3*\stepx,1.3*\stepy)  coordinate (p1);
\path (0,0)++(3.3*\stepx,2.3*\stepy)  coordinate (p2);
\draw[-stealth,my_cp_col5, line width=\mylinewidth, opacity=0.9] (p1) -- (p2) ;

%****** Going right - down  ********
\path (0,0)++(3.3*\stepx,2.5*\stepy)   coordinate (p1);
\path (0,0)++(4.3*\stepx,2.5*\stepy) coordinate (p2);
\path (0,0)++(4.3*\stepx,1.5*\stepy) coordinate (p3);
\draw[-stealth,my_cp_col5, line width=\mylinewidth, opacity=0.9,rounded corners = 0.2*\unit] (p1) -- (p2) -- (p3) ;

%****** Going up - down
\path (0,0)++(4.3*\stepx,1.1*\stepy)  coordinate (p1);
\path (0,0)++(4.3*\stepx,0.3*\stepy) coordinate (p2);
\draw[-stealth,my_cp_col5, line width=\mylinewidth, opacity=0.9] (p1) -- (p2) ;




\end{tikzpicture}


==> figures/fig_1_source_tikz.tex <==
% !TEX root = ../compiler_paper.tex



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%% COLORS %%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%-- Viridis Color Palette
\definecolor{my_cp5_col1}{RGB}{253, 231, 37}
\definecolor{my_cp5_col2}{RGB}{180, 222,44}
\definecolor{my_cp5_col3}{RGB}{94, 201, 98}
\definecolor{my_cp5_col4}{RGB}{33, 145, 140}
\definecolor{my_cp5_col5}{RGB}{59, 82, 139}
\definecolor{my_cp5_col6}{RGB}{68, 1, 84}

%--- Secondary Viridis Color Palette  (More pastel like)
\definecolor{my_cp2_col1}{RGB}{255,255,217}
\definecolor{my_cp2_col2}{RGB}{237,248,177}
\definecolor{my_cp2_col3}{RGB}{199,233,180}
\definecolor{my_cp2_col4}{RGB}{127,205,187}
\definecolor{my_cp2_col5}{RGB}{65,182,196}
\definecolor{my_cp2_col6}{RGB}{29,145,192}
\definecolor{my_cp2_col7}{RGB}{34,94,168}
\definecolor{my_cp2_col8}{RGB}{37,52,148}
\definecolor{my_cp2_col9}{RGB}{8,29,88}





%%------------- Scaling Factor ---------

\def \myfactor {0.65}
\def \unit  {\myfactor cm}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%% Definition of Blocks %%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% Definition of a block for block diagrams
\tikzstyle{block} = [ rectangle,
                      minimum width = \unit,
                      minimum height = \unit,
                      fill = gray,
                      draw = black,
                      text = black]

% Control the color and size of filter blocks
\tikzstyle{filter} = [block,
                      minimum width  = 3.5*\unit,
                      minimum height = 1.5*\unit,
                      fill = my_cp2_col7,
                      fill opacity=1,
                      text opacity=1]


% Control the color and size of nonlinearity blocks
\tikzstyle{nonlinearityb} = [ filter,
minimum width  = 3.5*\unit,
                             fill = my_cp2_col3,
                             fill opacity=1,
                             text opacity=1,
rounded corners = 0*\unit]


% Control separation between blocks
\def\deltainput     {(0,0)}
\def\deltalayer     {3}
\def\deltasigmab     {( 3.5, 0.0)}


% Filters in the input layer
%
\def \one   {$\textcolor{my_cp2_col2}{\displaystyle{  \boldsymbol{w}_{1}^{(1,0)}\ast f }}$}
%
\def \two   {$\textcolor{my_cp2_col2}{\displaystyle{\boldsymbol{w}_{2}^{(1,0)}\ast f    }}$}








%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%% BEGIN FIGURE CODE %%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

{\fontsize{10}{10}\selectfont\begin{tikzpicture}[scale = \myfactor]

  \pgfdeclarelayer{bg}     % declare background layer
  \pgfsetlayers{bg,main}   % set the order of the layers (main is the standard layer)

  % Putting a reference point to draw the structure
  \node (input) [rectangle, minimum width = 0.1*\unit] {};



%%-------------------------------------------------------
%%------------- L A Y E R  0 : INPUT LAYER --------------
%%-------------------------------------------------------

%----- Filters -----

% Filter 1
  \path (input.east)  ++ \deltainput node [filter]     (L1F1) {\one};
% Filter 2
%  \path (L1F1) ++ (0,-\deltalayer) node [filter]       (L1F2) {\two};
% Filter 3
  \path (L1F1) ++ (0,-1.3*\deltalayer) node [filter]       (L1F3) {\two};

%----- Point-wise nonlinearities -----
% Nl1
  \path (L1F1.east) ++ \deltasigmab node [nonlinearityb] (L1Nl1)      {
  \textcolor{my_cp5_col6}{
   $
    \displaystyle h_{1}^{(1)}= \eta\left( g_{1}^{(1)}\right)
   $
   }
    };
% Nl2
   \path (L1F3.east) ++ \deltasigmab node [nonlinearityb] (L1Nl3)      {
   \textcolor{my_cp5_col6}{
   	$
   	\displaystyle h_{2}^{(1)} = \eta\left( g_{2}^{(1)} \right)
   	$
    }
   };



 %%-------------------------------------------------------
 %%--------------------- L A Y E R  1  -------------------
 %%-------------------------------------------------------

  %------- First block of filters, index i=1

  % Filter 1
  \path (L1Nl1) ++ (2*\deltalayer,0.3*\deltalayer) node [filter]       (L2F1) {
  	\textcolor{my_cp2_col2}{
  		$
  		\boldsymbol{w}_{1}^{(2,1)}
  		\ast
  		h_{1}^{(1)}
  		$
  		}
  	};
  % Filter 2
  %\path (L1Nl1) ++ (2*\deltalayer,0) node [filter]       (L2F2) {\one};
  % Filter 3
  \path (L1Nl1) ++ (2*\deltalayer,-0.3*\deltalayer) node [filter]       (L2F3) {
  	\textcolor{my_cp2_col2}{
  		$
  		\boldsymbol{w}_{1}^{(2,2)}
  		\ast
  		h_{2}^{(1)}
  		$
  	    }
  	};


  %------- Second block of filters, index i=2

  % Filter 1
  \path (L1Nl3) ++ (2*\deltalayer,0.3*\deltalayer) node [filter]       (L2bF1) {
  	\textcolor{my_cp2_col2}{
  		$
  		\boldsymbol{w}_{2}^{(2,1)}
  		\ast
  		h_{1}^{(1)}
  		$
  	}
  	};
  % Filter 2
  %\path (L1Nl3) ++ (2*\deltalayer,0) node [filter]       (L2F2) {\one};
  % Filter 3
  \path (L1Nl3) ++ (2*\deltalayer,-0.3*\deltalayer) node [filter]       (L2bF3) {
  	  	\textcolor{my_cp2_col2}{
  	  		$
  	  		\boldsymbol{w}_{2}^{(2,2)}
  	  		\ast
  	  		h_{2}^{(1)}
  	  		$
  	  	}
  	};




  %%%------------------------------------------------
  %%%--------- O P L U S   S Y M B O L S  -----------
  %%%------------------------------------------------

  \path (L2F1) ++ (1.2*\deltalayer, -0.25*\deltalayer) node [scale=2] (oplusa){\textcolor{black}{$\oplus$}};

  \path (L2bF1) ++ (1.2*\deltalayer, -0.25*\deltalayer) node [scale=2] (oplusb){\textcolor{black}{$\oplus$}};
  %\path (L2F1) ++ (-4, 0) node [scale=1]  (x) {\textcolor{black}{$\bbx$}};





  %----- Point wise nonlinearities -----
  % Nl1
  \path (oplusa.east) ++ \deltasigmab node [nonlinearityb] (L2Nl1)      {
  \textcolor{my_cp5_col6}{
  	$
  	h_{1}^{(2)} = \eta\left( g_{1}^{(2)} \right)
  	$
        }
  };
  % Nl2
  \path (oplusb.east) ++ \deltasigmab node [nonlinearityb] (L2Nl3)      {
  \textcolor{my_cp5_col6}{
  	$
  	h_{2}^{(2)} = \eta\left( g_{2}^{(2)} \right)
  	$
   }
  };


  % Oplus Symbols Again
  \path (L2Nl1) ++ (\deltalayer, -0.65*\deltalayer) node [scale=2] (oplusc){\textcolor{black}{$\oplus$}};






  %%------------------------------------------------
  %%----- Arrows going from x to the architecture -----------
  %%------------------------------------------------

  \path (L1F1) ++ (-1.2*\deltalayer, -0.65*\deltalayer) node [scale=1]  (x) {$f$};

  \path[draw, -stealth] (x.east) -- (L1F1.west);
  \path[draw, -stealth] (x.east) -- (L1F3.west);
  %\path[draw, -stealth] (x.east) -- (L3F1.west);




   %%------------------------------------------------
   %%---------- Arrows between Blocks  -----------
   %%------------------------------------------------

  \path[draw, -stealth] (L1F1.east) --  node [above] {$g_{1}^{(1)}$} (L1Nl1.west);

  \path[draw, -stealth] (L1F3.east) --  node [above] {$g_{2}^{(1)}$} (L1Nl3.west);


  \path[draw, -stealth] (L1Nl1.east) --  node [above] {} (L2F1.west);
  \path[draw, -stealth] (L1Nl1.east) --  node [above] {} (L2bF1.west);

  \path[draw, -stealth] (L1Nl3.east) --  node [above] {} (L2F3.west);
  \path[draw, -stealth] (L1Nl3.east) --  node [above] {} (L2bF3.west);


  \path (oplusa) + (-0.28,0) coordinate (c1);
  \path[draw, -stealth] (L2F1.east) --  node [above] {} (c1);
  \path[draw, -stealth] (L2F3.east) --  node [above] {} (c1);

  \path (oplusb) + (-0.28,0) coordinate (c1);
  \path[draw, -stealth] (L2bF1.east) --  node [above] {} (c1);
  \path[draw, -stealth] (L2bF3.east) --  node [above] {} (c1);


  \path (oplusa) + (0.28,0) coordinate (c1);
  \path[draw, -stealth] (c1) --  node [above] {$g_{1}^{(2)}$} (L2Nl1.west);

  \path (oplusb) + (0.28,0) coordinate (c1);
  \path[draw, -stealth] (c1) --  node [above] {$g_{2}^{(2)}$} (L2Nl3.west);


  \path (oplusc) + (0,0.28) coordinate (c1);
  \path[draw, -stealth] (L2Nl1.east) --  node [above] {} (c1);

  \path (oplusc) + (0,-0.28) coordinate (c1);
  \path[draw, -stealth] (L2Nl3.east) --  node [above] {} (c1);



  %%---------- Output Signal ----------

  \path (oplusc.east) ++ (1, 0) node [scale=1]  (yout) {\textcolor{black}{$f_{out}$}};


  \path (oplusc) + (0.2,0) coordinate (c1);
  \path[draw, -stealth] (c1) --  node [above] {} (yout);


%%------------------------------------------
  %%----- Light shades to signify layer groups --------
  %%------------------------------------------

  \begin{pgfonlayer}{bg}
      % Shading for Layer 1
      \path (L1F3.west |- L1F3.south) ++ (-0.4,-1.3)
           node [filter, anchor = south west,
                 fill = black!5,
                 %minimum width  = 10.75*\unit,
                 minimum width  = 9.85*\unit,
                 minimum height = 8*\unit,]
        (layer)
        {};
      % Shading for Layer 2
        \path (L2bF3.west |- L2bF3.south) ++ (-0.4,-0.4)
           node [filter, anchor = south west,
                 fill = black!5,
                 %minimum width  = 10.75*\unit,
                 minimum width  = 12.5*\unit,
                 minimum height = 8*\unit,]
        (layer)
        {};
    \end{pgfonlayer}




\end{tikzpicture}}


==> v12/sec_app_gphon_sp.tex <==
%!TEX root =../compiler_paper.tex





%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%   S E C T I O N    %%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\section{Numerical Experiments: Learnable Filters in Gphon-SP}
\label{sec_alg_rkhs_nn}




As discussed in Section~\ref{subsubsec_gphonsp}, Gphon-SP is directly connected to RKHS theory and to algebraic signal models defined on RKHS. Consequently, it provides a concrete setting where the results presented in Section~\ref{sec_rkhs_filt_rep_asp_filt} can be directly applied. In what follows, we elaborate on these implications in detail.


































\blue{
**********************************************\\
******  AlejandroPM:  I AM HERE  *************\\
**********************************************
}



Additionally, one can leverage $T_{W}$ to define a convolutional signal processing model defined \textit{on} $W(u,v)$~\cite{gphon_pooling_c,gphon_pooling_j}. This can be done with the ASM $(\mbC[t],L_{2}([0,1]),\rho_{W})$, where $\mbC[t]$ is the polynomial algebra with independent variable $t$, $L_{2}([0,1])$ is the set of square integrable functions on $[0,1]$ with the Lebesgue measure, and $\rho_{W}: \mbC[t]\to\ccalB(L_{2}([0,1]))$ is the homomorphism that maps $t$ into $T_{W}$. Then, if $p(t)$ is a polynomial, the action of $\rho_{W}$ can be written as
%
%
%
\begin{equation}
\rho_{W}\left( p(t) \right)
       \left\lbrace 
              \boldsymbol{x}
       \right\rbrace
            =
            p\left(
                 T_{W}
             \right)
                    \left\lbrace 
                             \boldsymbol{x}
                   \right\rbrace
            .
\end{equation}
%
%
%




























==> v12/sec_background_rkhs.tex <==
%!TEX root =../compiler_paper.tex





%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%% SECTION %%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\section{Basic Preliminaries}
\label{sec_appendix_basic_prelim}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%% Sub - Section %%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Auxiliary Results}


Now, we turn our attention to results where we have a general description of how kernels can be built from certain types of functions and their intricate relationship with exponential maps. To do so, we start considering the following definitions.






%%-------------------------------------
%%------------ THEOREM -----------------
%%-------------------------------------

\begin{theorem}(Theorem 2.4~\cite{paulsen2016introduction})
\label{thm_K_from_basis_general}
Let $\ccalH(K)$ be an RKHS on $\ccalT$ with reproducing kernel $K$. If $\{ \boldsymbol{e}_{s}: s\in\ccalS \}$ is an orthonormal basis for $\ccalH$, then
%
%
%
\begin{equation}
K(u,v)
   =
    \sum_{i=1}^{\infty}
            \boldsymbol{e}_{i}(u)
            \overline{\boldsymbol{e}_{i}(v)}
            ,
\end{equation}
%
%
%
where this series converges pointwise.
\end{theorem}

%%-------- End of Theorem ----------------






As one can expect, specific attributes of $K(u,v)$ influence the norm associated with $\ccalH (K)$. In the case of kernels obtained from symbols and the box product, this can be formalized in the following theorem.



%%---------------------------------------------------
%%------------ T H E O R E M -----------------
%%--------------------------------------------------

\begin{theorem}[Theorem 11.3~\cite{paulsen2016introduction}]
\label{thm_kernel_from_box_prod}
%
Let $\ccalT$ be a set, let $(\ccalU, \mu)$ be a measure space, let $S(u,v): \ccalT \times \ccalU \to \mbC$ be square integrable in the $v$ variable and let $K: \ccalT\times \ccalT \to \mbC$ be the kernel function given by $K(u,z) = \left( S\square S^{\ast} \right)(u,z) $. Then $\left\lbrace  T_{S}\left\lbrace \boldsymbol{g} \right\rbrace: \boldsymbol{g}\in L^{2}(\ccalY,\mu)  \right\rbrace = \ccalH (K)$ and for $\boldsymbol{f}\in\ccalH (K)$ we have that
%
%
%
\begin{equation}
 \left\Vert 
       \boldsymbol{f}
 \right\Vert_{\ccalH (K)}
       =
       \inf 
           \left\lbrace 
                 \Vert \boldsymbol{g} \Vert_{2}
                      :
                       \boldsymbol{f} = T_{S} \{ \boldsymbol{g} \}
           \right\rbrace
           .
\end{equation}
%
%
%
\end{theorem}

%%---------- End of Theorem ------------











%%-------------------------------------
%%---------- DEFINITION ---------------
%%-------------------------------------

\begin{definition}[~\cite{paulsen2016introduction}]\label{def_neg_def_func}
A function $\psi: \ccalX\times\ccalX \to \mbC$ is called conditionally negative definite if and only if, given $x_1, \ldots, x_n \in \ccalX$ and $\alpha_1, \ldots, \alpha_n \in \mbC$ such that $\sum_{j=1}^{n}\alpha_j = 0$, we have
%
%
%
\begin{equation}
\sum_{i,j=1}^{n}
       \overline{\alpha}_{i}\alpha_{j}
             \psi (x_i , x_j) 
             \leq 0
             .
\end{equation}
%
%
%
The function $\psi$ is called negative definite provided that this later inequality is met for all $\alpha_1, \ldots, \alpha_n \in \ccalX$.
\end{definition}

%%-------- End of Definition ----------




%%-------------------------------------
%%---------- DEFINITION ---------------
%%-------------------------------------

\begin{definition}[~\cite{paulsen2016introduction}]\label{def_neg_def_adjnt}
A conditionally negative definite function $\psi: \ccalX\times\ccalX \to \mbC$ is called self-adjoint provided that $\psi (y,x) = \overline{\psi (x,y)}$ and symettric provided that $\psi (y,x) = \psi (x,y)$.
\end{definition}

%%-------- End of Definition ----------


With Definitions~\ref{def_neg_def_func} and~\ref{def_neg_def_adjnt} at hand, we are ready to the so called Schoenberg's generator theorem, which leverages conditional negative definite functions and the exponential map to build families of kernels.


%%-------------------------------------
%%------------ THEOREM -----------------
%%-------------------------------------

\begin{theorem}(Theorem 9.7~\cite{paulsen2016introduction})
\label{thm_gen_kernel_exp}
The function $\psi: \ccalX \times \ccalX \to \mbC$ is a self-adjoint conditionally negative definite function if and only if the function $K_{t} = e^{-t\psi}$ is a kernel function for all $t>0$.
\end{theorem}

%%-------- End of Example ----------------


An interesting aspect of Theorem~\ref{thm_gen_kernel_exp} is that, it provides a concrete formula to generate kernels from negative definite functions exploiting the exponential map. This attribute endows the family of kernels $K_t$ with the structure of a semigroup and it formally allows one to capture time varying signals that are formally associated to an RKHS for each value of time. A similar result is derived in~\cite{paulsen2016introduction} considering the parametrization given by $L_t = t/(t+\psi(x,y))$ -- see Appendix~\ref{sec_appendix_basic_prelim}.







%%-------------------------------------
%%------------ THEOREM -----------------
%%-------------------------------------

\begin{theorem}(Theorem 9.9~\cite{paulsen2016introduction})
Let $\psi: \ccalX \times \ccalX \to \mbC$ with $\mathfrak{Re}\{ \psi(x,y) \}\geq 0$ for all $x,y\in\ccalX$. Then $\psi$ is self-adjoint and conditionally negative definite if and only if the function $L_t = t/(t+\psi(x,y))$ is a kernel function for all $t>0$.
\end{theorem}

%%-------- End of Example ----------------








%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%% Sub - Section %%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Relationship between inner products}
\label{sub_sec_Ts_Tk_relationship}

Since the functions $\boldsymbol{\varphi}_i$ constitute an orthonormal basis in $L_{2}(\ccalT,\mu)$, we can compute the inner product $\langle , \rangle_{\ccalH(K)}$ as follows
%
%
%
\begin{equation}
\left\langle 
   \boldsymbol{f}
   ,
   \boldsymbol{g}
\right\rangle_{\ccalH(K)}
=
\left\langle 
      \sum_{i}\langle 
                    \boldsymbol{f}
                    ,
                    \boldsymbol{\varphi}_i
              \rangle_{L_{2}}      
              \boldsymbol{\varphi}_i
       ,
        \sum_{i}\langle 
                    \boldsymbol{g}
                    ,
                    \boldsymbol{\varphi}_i
              \rangle_{L_{2}}      
              \boldsymbol{\varphi}_i
\right\rangle_{\ccalH(K)}
,
\end{equation}
%
%
%
then rearranging terms and exploiting the linearity properties of the inner products we have that
%
%
%
\begin{equation}
\left\langle 
   \boldsymbol{f}
   ,
   \boldsymbol{g}
\right\rangle_{\ccalH(K)}
=
\sum_{i=1}^{\infty}
   \left\Vert 
         \boldsymbol{\varphi}_i
   \right\Vert_{\ccalH(K)}^{2}
         \langle
             \boldsymbol{f}
             ,
             \boldsymbol{\varphi}_i
         \rangle_{L_2} 
          \overline{\langle
             \boldsymbol{g}
             ,
             \boldsymbol{\varphi}_i
         \rangle}_{L_2}   
         .
\end{equation}
%
%
%
To find the value of
%
%
$
 \left\Vert 
         \boldsymbol{\varphi}_i
   \right\Vert_{\ccalH(K)}^{2}
$
%
%
we take into account that
%
%
%
\begin{equation}
\boldsymbol{\varphi}_{i}(v)
=
\left\langle
   \boldsymbol{\varphi}_{i}
   ,
   \boldsymbol{k}_{v}
\right\rangle_{\ccalH(K)}
=
\left\langle
      \boldsymbol{\varphi}_{i}
      ,
      \sum_{j=1}^{\infty}
          \sigma_{j}
          \boldsymbol{\varphi}_{j}
          \overline{\boldsymbol{\varphi}_{j}(v)}
\right\rangle_{\ccalH(K)}
,
\end{equation}
%
%
%
which leads to
%
%
%
\begin{equation}\label{eq_norm_squared_in_HK_varphi}
\boldsymbol{\varphi}_{i}(v)
     =
     \sigma_{i}
     \boldsymbol{\varphi}_{i}(v)
     \left\Vert
          \boldsymbol{\varphi}_{i}
     \right\Vert_{\ccalH(K)}^{2}
     \Rightarrow
     \left\Vert
          \boldsymbol{\varphi}_{i}
     \right\Vert_{\ccalH(K)}^{2}
     =
     \frac{1}{\sigma_i}
     .
\end{equation}
%
%
%
We can see then that $\boldsymbol{e}_i = \boldsymbol{\varphi}_{i}\sqrt{\sigma_i}$ constitutes an orthonormal basis for $\ccalH(K)$.









==> v12/sec_convolutional_filtering_in_rkhs.tex <==
%!TEX root =../compiler_paper.tex





%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%% SECTION %%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\section{Convolutional Filtering in RKHS}
\label{sec_conv_filt_rkhs}


%%-----------------------------------
%%------------ FIGURE ---------------
%%-----------------------------------

\begin{figure}
        \centering
        \input{figures/asp_diagrams/fig2_tikz_source_b.tex} 
        \caption{Pictorial representation of a generic algebraic signal model (ASM) $(\ccalA, \ccalM, \rho)$. Filters are elements of the algebra $\ccalA$ while the signals are the elements of the vector space $\ccalH$. The homomorphism, $\rho$, translates the abstract filters in $\ccalA$ into concrete operators in $\ccalB(\ccalH)$ that act on the signals in $\ccalH$. The symbol $\ccalB(\ccalH)$ indicates the space of operators from $\ccalH$ onto itself.}
        \label{fig_asp_model}
\end{figure}

%%--------- End of Figure -----------




In this section, we study the algebraic structure of convolutional filters associated with an arbitrary RKHS. Let us recall that any convolutional signal processing model is determined by the triplet $(\ccalA, \ccalM,\rho)$, where $\ccalA$ is an unital algebra, $\ccalM$ is a vector space and $\rho:\ccalA \to \ccalB(\ccalM)$ is a homomorphism, where $\ccalB (\ccalM)$ is the set of bounded operators from $\ccalM$ onto itself~\cite{algSP0,algSP1,algnn_nc_j}. The filters are the elements in $\ccalA$ while the signals are the elements of $\ccalM$. The homomorphism $\rho$ translates the abstract filters in $\ccalA$ into concrete operators that act directly on the information in $\ccalM$. In this framework, we can represent a wide variety of convolutional signal models used such as discrete time signal processing~\cite{algSP1}, discrete space models with symmetric shift operators~\cite{algSP2}, signal processing on 2D spatial hexagonal lattices~\cite{algSP6}, models on general lattices~\cite{puschel_asplattice}, signal processing on sets~\cite{puschel_aspsets}, among others~\cite{algSP7}. 


In the following subsection, we focus our attention on building algebraic models of the type $(\ccalA,\ccalM,\rho)$, where $\ccalA$ is built from the structural properties of an RKHS. 



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%% sub- Section %%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Algebras from RKHS}

Let $K(u,v)$ be the reproducing kernel of the RKHS $\ccalH$. From previous definitions, we know that $K(u,v) = \boldsymbol{k}_{v}(u)$, i.e. $\boldsymbol{k}_{v}(u)$ is a function whose independent variable is $u$ and which is associated to $v\in\ccalT$. Additionally we have $\boldsymbol{k}_{v}\in\ccalH$. Now we proceed to state how algebras can be obtained from RKHS formally. 



%%------------------------------------------
%%------------ T H E O R E M ---------------
%%------------------------------------------

\begin{theorem}\label{thm_general_A_rkhs}

Let $\ccalH\subset\ccalF(\ccalT,\mbF)$ be a RKHS with reproducing kernel $K(u,v)$. Let $\ccalA_{\ccalH(K)}$ be the set given by
%
%
%
\begin{equation}\label{eq_A_rkhs_gen}
\ccalA_{\ccalH(K)} 
    =
    \left\lbrace 
       \left.
           \sum_{i\in\ccalI}\alpha_{i}\boldsymbol{k}_{i}(t)
       \right\vert 
           \boldsymbol{k}_{i}(t) = K(t,i),
           ~\ccalI\subset\ccalT~\text{countable}
    \right\rbrace
    ,
\end{equation}
%
%
%
and let $\bullet: \ccalA_{\ccalH} \times \ccalA_{\ccalH} \to \ccalA_{\ccalH}$ be the product map given by
%
%
%
\begin{equation}\label{eq_A_rkhs_gen_prod}
    \left( 
     \sum_{i\in\ccalI}\alpha_{i}\boldsymbol{k}_{i}(t)
\right)
      \bullet
\left( 
     \sum_{j\in\ccalJ}\beta_{j}\boldsymbol{k}_{j}(t)
\right)  
      =
      \sum_{i,j}\alpha_{i}\beta_{j} \boldsymbol{k}_{\theta(i,j)}(t)
      ,
\end{equation}
%
%
%
where $\ccalJ\subset\ccalT$ is countable and $\theta: \ccalT \times \ccalT \to \ccalT$ satisfies that 
%
%
%
\begin{equation}
\theta\left(  
         \theta\left(
                   i,j
               \right)
               ,
               \ell
      \right)
             =
              \theta\left( 
                         i
                          ,
                         \theta\left( 
                                   j,\ell
                                \right)
                    \right)
                    .
\end{equation}
%
%
%
If there exists an element $\delta\in\ccalT$ such that 
%
%
%
\begin{equation}
 \theta (\delta,u) = \theta (u,\delta) = u\quad \forall~u\in\ccalT   
 ,
\end{equation}
%
%
%
then $\ccalA_{\ccalH}$ is an algebra when endowed with the product $\bullet$.
\end{theorem}

\begin{proof}  See Appendix~\ref{proof_thm_general_A_rkhs}  \end{proof}

%%------------ End of Theorem --------------



Theorem~\ref{thm_general_A_rkhs} states general conditions that will allow us to build algebras from RKHS, and it is meant to be general to highlight the richness of the algebraic models that can be derived in this context. In the following examples, we consider particular instantiations of Theorem~\ref{thm_general_A_rkhs}.



%%-----------------------------------
%%----------- EXAMPLES --------------
%%-----------------------------------

\begin{example}\label{ex_rkhs_pw_2}\normalfont
%
In the context of Example~\ref{exa_rkhs_pw} we have that $\boldsymbol{k}_{v_1}\ast \boldsymbol{k}_{v_2} = \boldsymbol{k}_{v_3}$, where $\ast$ denotes the traditional ordinary convolution of functions on the real line. In particular, we have $v_{3} = v_{1} + v_{2}$. Then, we can exploit the usual convolution to build an algebra, $\ccalA_{\ccalH}$, as in~\eqref{eq_A_rkhs_gen} with the algebra product $\bullet$ is given according to
%
%
%
\begin{multline}\label{eq_A_rkhs_prod_1}
\left( 
     \sum_{i\in\ccalI}\alpha_{i}\boldsymbol{k}_{i}(t)
\right)
      \bullet
\left( 
     \sum_{j\in\ccalJ}\beta_{j}\boldsymbol{k}_{j}(t)
\right)  
      =
      \sum_{i\in\ccalI,j\in\ccalJ}\alpha_{i}\beta_{j} \boldsymbol{k}_{i}(t)\ast \boldsymbol{k}_{j}(t)
      \\
      \sum_{i,j}\alpha_{i}\beta_{j} \boldsymbol{k}_{i+j}(t)
      .
\end{multline}
%
%
%
This is, we consider
%
%
$
 \theta (i,j) = i + j
 ~\text{and}~
\delta = 0
  .
$
%
%
Here $\ccalJ$ is also a countable set $\ccalJ\subset\ccalT$. Since the sum of two countable sums is again a countable sum and the scalar multiplication of one of these sums is again a countable sum in terms of the $\boldsymbol{k}_{v}$, $\ccalA_{\ccalH}$ is a vector space. Note that the structure of $\ccalA_{\ccalH}$ as a vector space is not identical to that of $\ccalH$. The product indicated in~\eqref{eq_A_rkhs_prod_1} is associative since the ordinary convolution operation is associative as well. Additionally, $\ccalA_{\ccalH}$ has a unit element given by $\boldsymbol{k}_{0}(t) = K(t,0)$. To see this note that $\boldsymbol{k}_{0}(t)\ast \boldsymbol{k}_{i}(t) = \boldsymbol{k}_{i}(t)$ for all $i\in\ccalT$.
%
\end{example}

%%------- End of Example ------------







%%--------------------------------------------------------
%%------------------ R E M A R K --------------------
%%--------------------------------------------------------

\begin{remark}\normalfont
As pointed out in~\cite[p.~396]{wainwright2019high}, the framework of RKHS with Mercer kernels can be interpreted as a tool that allow us to embed the domain of the signals, $\ccalT$, into $\ell^{2}(\mbN)$ when considering the map
%
%
%
\begin{equation}\label{eq_rkhs_as_feature_map}
t  
  \mapsto
              \boldsymbol{\Phi}(t)
               =
                 \left( 
                        \sqrt{\sigma_1}\boldsymbol{\varphi}_{1}(t)
                        ,
                        \sqrt{\sigma_2}\boldsymbol{\varphi}_{2}(t)
                        ,
                        \sqrt{\sigma_3}\boldsymbol{\varphi}_{3}(t)
                        ,
                       \ldots
                 \right)
                 ,
\end{equation}
%
%
%
where the associated reproducing kernel, $K$, is given by~\eqref{eq_mercer_K_decomp}. This is, the RKHS provides us naturally with a \textit{feature map} given by~\eqref{eq_rkhs_as_feature_map}, where additionally we have that $\Vert  \boldsymbol{\Phi}(t)\Vert^{2}_{\ell^{2}(\mbN)}=K(t,t)$ and $\langle  \boldsymbol{\Phi}(t_{1}) ,  \boldsymbol{\Phi}(t_{2})\rangle_{\ell^{2}(\mbN)}=K(t_{1}, t_{2})$. Such embedding, while convienient, does not incorporate the symmetries of $\ccalT$, and this is precisely what we can achieve with the algebra $\ccalA_{\ccalH(K)}$ in Theorem~\ref{thm_general_A_rkhs} for the properties of $\ccalT$ are embedded in the product operation of $\ccalA_{\ccalH(K)}$. This particular attribute of $\ccalA_{\ccalH(K)}$ enhance the ability to perform scalable learning. For example, if $\ccalT$ has the structure of a group, $\theta (\cdot,\cdot)$ can be chosen to be the group product, and $\delta$ is the group identity element -- we elaborate more about this scenario in the next subsection.
%
\end{remark}

%%------------------ End of Remark ----------------




Before we turn our attention to another family of algebras, we emphasize that the ASM associated with $\ccalA_{\ccalH(K)}$ that we consider is 
%
%
%
\begin{equation}\label{eq_rkhs_asm_standard}
\left( 
      \ccalA_{\ccalH(K)}
      ,
      \ccalH(K)
      ,
      \rho_{\ccalH(K)}
\right)
,
\end{equation}
%
%
%
where the homomorphism $\rho$ translates the action of the filter 
%
%
$
\boldsymbol{h}
         =
          \sum_{i\in\ccalI}h_{i}\boldsymbol{k}_{i}(t)
$
%
%
on the signal 
%
%
$
\boldsymbol{x}
         =
          \sum_{j\in\ccalJ}x_{j}\boldsymbol{k}_{j}(t)
$
%
%
according to
%
%
%
\begin{multline}\label{eq_rho_in_rkhs_a}
\rho_{\ccalH(K)}
       \left(
             \boldsymbol{h}
      \right)
      \left\lbrace 
             \boldsymbol{x}
      \right\rbrace       
=      
\rho\left( 
          \sum_{i\in\ccalI}h_{i}\boldsymbol{k}_{i}(t)
    \right)
            \left\lbrace 
                    \sum_{j\in\ccalJ}x_{j}\boldsymbol{k}_{j}(t)
            \right\rbrace
\\           
= 
\left( 
          \sum_{i\in\ccalI}h_{i}\boldsymbol{k}_{i}(t)
    \right)
           \bullet
                  \left(
                         \sum_{j\in\ccalJ}x_{j}\boldsymbol{k}_{j}(t)
                  \right)
\\                  
=
\sum_{i\in\ccalI,j\in\ccalJ}h_{i}x_{j}\boldsymbol{k}_{\theta (i,j)}
.
\end{multline}
%
%
%
Notice that one can build multiple ASMs by keeping the same algebra, $\ccalA_{\ccalH(K)}$, while choosing an arbitrary vector space. However, in our discussion we focus on $\ccalH(K)$ as the vector space of signals when using $\ccalA_{\ccalH(K)}$.




Now we introduce another general algebra that can be built from those RKHS that are linked to integral operators. Although $\ccalA_{\ccalH(K)}$ in~\eqref{eq_A_rkhs_gen} will have the central role in our analysis, the algebra we will introduce next will allow us to build signal processing models where one can link the attributes of the filtering with the decomposition of the signals in terms of the eigenvectors of the reproducing kernel.  




%%--------------------------------------------
%%---------------- THEOREM -------------------
%%--------------------------------------------

\begin{theorem}
\label{thm_alg_RKHS_box_prod}
%
Let $K$ be a Mercer kernel on $\ccalT\times\ccalT$ and let $\mu$ be a finite Borel measure on $\ccalT$. Let $\boldsymbol{\varphi}_i$ and $\sigma_i$ the eigenvectors and eigenvalues in the spectral decomposition of the integral operator $T_{K}: L^{2}(\ccalT,\mu)\to L^{2}(\ccalT,\mu)$ -- see Theorem~\ref{thm_mercer} --, and
%
%
$
K(u,v) = 
        \sum_{i}
             \sigma_{i}
             \boldsymbol{\varphi}_{i}(u)
             \boldsymbol{\varphi}_{i}(v)
             .
$
%
%
%
Let $\ccalA_{K}$ be the set given by
%
%
%
\begin{equation}\label{eq_A_rkhs_box_1}
\ccalA_{K} 
   =
   \left\lbrace 
      \left.
          \sum_{r=0}^{R}a_{r}K^{\square r}
      \right\vert 
          a_{r}\in\mbF,
          ~R\in\mbN
   \right\rbrace
   ,
\end{equation}
%
%
%
where $K^{\square r}$ indicates the $r$-times box product of $K$ with itself. Let $\bullet: \ccalA_{K} \times \ccalA_{K} \to \ccalA_{K}$ be given by
%
%
%
\begin{equation}\label{eq_A_rkhs_box_2}
\left(
    \sum_{r=0}^{R}a_{r}K^{\square r}
\right)
     \bullet
\left(
    \sum_{\ell=0}^{L}b_{\ell}K^{\square\ell}
\right)  
     =
     \sum_{r=0, \ell=0}^{R,L}
           a_{r}b_{\ell}
           K^{\square (r+\ell)}
           .
\end{equation}
%
%
%
Then, $\ccalA_{K}$ is an algebra endowed with the product $\bullet$ and identity element $1_{\ccalA_{K}}$ given by
%
%
%
\begin{equation}\label{eq_A_rkhs_box_3}
1_{\ccalA_{K}}
=
K^{\square 0}
\equiv
    \sum_{i=1}^{\infty}
         \boldsymbol{\varphi}_{i}(u)
         \boldsymbol{\varphi}_{i}(v)
         .
\end{equation}
%
%
%
Additionally, the function
%
%
$
\boldsymbol{q}_{v}(K\vert\square)
=
\left(
p 
    \left(
             K\vert\square
    \right) 
    \square
    K
\right)(u,v)   
$
%
%
obtained by fixing the value of the variable $v$ in the expression
%
%
$
\left(
p 
    \left(
             K\vert\square
    \right) 
    \square
    K
\right)(u,v)   
,
$
%
%
belongs to $\ccalH(K)$.
\end{theorem}

\begin{proof} See Appendix~\ref{proof_thm_alg_RKHS_box_prod} \end{proof}

%%-------------- End of Theorem --------------



\noindent We represent the generic polynomials in $\ccalA_{K}$ by $p\left(K \vert \square\right)$. Then, we obtain the expression for $p\left( K \vert \square\right)$ by replacing the powers of the independent variable in $p$ -- an ordinary polynomial -- with powers on $K$ considering the box product, $\square$. For instance, if $p(t)= 1 + t + t^2$, then $p(K\vert\square)= 1_{\ccalA_{K}}+ K + K^{\square 2}$. 


One of the interesting properties of $\ccalA_{K}$ is that certain subset are indeed elements of $\ccalH(K)$. This will allow us to develop convolutional models involving $\ccalA_{K}$ as the algebra and $\ccalH(K)$ as the vector space in an ASM. Due to the importance of this fact, we formalize it in the following result.




%%-----------------------------------------------------------
%%----------------  T H E O R E M  --------------------
%%-----------------------------------------------------------

\begin{theorem}\label{thm_Ak_subsets_in_HK}
%
Let $p(t)$ be a polynomial and let $\ccalA_{K}$ be as defined in Theorem~\ref{thm_alg_RKHS_box_prod} for an RKHS $\ccalH(K)$. If
%
%
$
\boldsymbol{q}_{v}(K\vert\square)
=
\left(
p 
    \left(
             K\vert\square
    \right) 
    \square
    K
\right)(u,v)   
$
%
%
is the function -- on the variable $u$ -- obtained by fixing the value of  ``$v$" in the expression
%
%
$
\left(
p 
    \left(
             K\vert\square
    \right) 
    \square
    K
\right)(u,v)  
\in\ccalA_{K} 
,
$
%
%
then
%
%
$
\boldsymbol{q}_{v}(K\vert\square)
\in
\ccalH(K)
$
%
%
and 
%
%
$
\left\langle 
                    \boldsymbol{q}_{v}(K\vert\square)
                    ,
                    \boldsymbol{x}
\right\rangle_{\ccalH(K)}
\in\ccalH(K)
$             
%
%  
with ``$v$" as the independent variable. Additionally, the map $\rho_{K}: \ccalA_{K} \to \ccalB(\ccalH(K))$ given by
%
%
%
\begin{equation}\label{eq_rho_Ak_Hk}
\rho_{K}
      \left( 
             p\left(
                    K\vert\square
                \right)
      \right)
             \left\lbrace 
                   \boldsymbol{x}
             \right\rbrace
             =
             \boldsymbol{y}(v)
             =
             \left\langle 
                     \boldsymbol{q}_{v}(K\vert\square)
                    ,
                    \boldsymbol{x}
             \right\rangle_{\ccalH(K)}
             ,
\end{equation}
%
%
% 
is a homomorphism.
\end{theorem}

\begin{proof} See Appendix~\ref{sub_sec_proof_thm_Ak_subsets_in_HK} \end{proof}

%%------------  E N D   of Theorem   -----------------




From the results in Theorem~\ref{thm_Ak_subsets_in_HK}, we can obtain the convolutional model
$(\ccalA_{K}, \ccalH(K), \rho_{K})$. While there could be multiple ways to build the homomorphism in an ASM involving $\ccalA_{K}$, the map in~\eqref{eq_rho_Ak_Hk} exhibits a natural connection with the ASM $(\mbC[t], L_{2}(\ccalT,\mu), \rho)$, where $\mbC[t]$ is the polynomial algebra and $\rho(t)=T_{K}$, with $T_{K}$ as in Theorem~\ref{thm_mercer}. Since this connection will be important for the discussion of RKHS convolutional models on graphons, we formalize it in the following theorem.




%%-----------------------------------------------------------
%%----------------  T H E O R E M  --------------------
%%-----------------------------------------------------------

\begin{theorem}\label{thm_alg_rkhs_vs_alg_classic}
%
Let $\ccalH(K)$ be an RKHS with Mercer reproducing kernel $K$. Let $T_{K}$ be as in Theorem~\ref{thm_mercer} and let $\ccalA_{K}$ be given according to Theorem~\ref{thm_alg_RKHS_box_prod}. Then, given the ASMs $(\ccalA_{K}, \ccalH(K), \rho_{K})$ and $(\mbC[t], L_{2}(\ccalT,\mu), \rho)$ with homorphisms $\rho_{K}$ given by~\eqref{eq_rho_Ak_Hk} and $\rho$ given by $\rho(t)=T_{K}$, we have that 
%
%
%
\begin{equation}\label{eq_thm_alg_rkhs_vs_alg_classic}
\rho\left( 
              p\left(
                      t
                \right)      
       \right)
             \left\lbrace 
                    \boldsymbol{x}
             \right\rbrace
             =
               \rho_{K}
                     \left(
                           p\left( 
                                    K \vert \square
                              \right)
                     \right)
                              \left\lbrace 
                                    \boldsymbol{x}
                             \right\rbrace
                             ,
\end{equation}
%
%
%
for all $\boldsymbol{x}\in\ccalH(K)$ and any polynomial $p(t)\in\mbC[t]$.
\end{theorem}

\begin{proof} See Appendix~\ref{proof_thm_alg_rkhs_vs_alg_classic} \end{proof}

%%-----------  E N D  of  Theorem  -------------------





Theorem~\ref{thm_alg_rkhs_vs_alg_classic} establishes a direct connection between the common diffusions in an ASM and the filtering operation in an RKHS. It is possible to see that 
%
%
$
\rho\left( 
              p\left(
                      T_{K}
                \right)      
       \right)
             \left\lbrace 
                    \boldsymbol{x}
             \right\rbrace
             \in
             \ccalH(K)
$
%
%
for any $\boldsymbol{x}\in\ccalH(K)\subset L_{2}(\ccalT,\mu)$, with $\ccalH(K)$ being a subclass of signals in $L_{2}(\ccalT, \mu)$. This is, $\ccalH(K)$ remains invariant under the action of 
%
%
$
\rho\left( 
              p\left(
                      T_{K}
                \right)      
       \right)
       .
$
%
%
This observation is key to quantify the effect of restricting the space of signals to be an RKHS. More specifically, we can say that if we require our space of signals to be an RKHS, we end up with a space that is invariant under the action of polynomial diffusions where $T_{K}$ is the shift operator. 

























%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%% SUB - SECTION %%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{RKHS algebras from Groups}
\label{sec_grsp_rkhs}

%%-----------------------------------
%%------------ FIGURE ---------------
%%-----------------------------------

\begin{figure*}
%
%--------- FIRST ROW ---------
%
\centering
       \begin{subfigure}{.32\linewidth}
	   \centering
          \includegraphics[width=1\textwidth]{./figures/kvs_on_sphere/fig_2.pdf} 
       \end{subfigure}
    	\begin{subfigure}{.32\linewidth}
		\centering
            \includegraphics[width=1\textwidth]{./figures/kvs_on_sphere/fig_4.pdf} 
\end{subfigure}
    	\begin{subfigure}{.32\linewidth}
		\centering
  \includegraphics[width=1\textwidth]{./figures/kvs_on_sphere/fig_3.pdf} 
\end{subfigure}
%
%
\caption{
Depiction of the functions in the RKHS on the sphere built from $\boldsymbol{k}_{v}(u)=\left\langle u, v\right\rangle^{4}$ with the group structure of $\mathsf{SO}(3)$ described in Example~\ref{ex_rkhs_on_sphere} . On the left, we show $\boldsymbol{x}(u)=\boldsymbol{k}_{v_1}(u)+\boldsymbol{k}_{v_2}(u)$ with $v_1 =[1,0,1](1/\sqrt{2})$ and $v_2 = [0,1,0]$. On the center we show $\boldsymbol{y}(u)=\boldsymbol{v_3}(u)$ with $v_3 =[1,1,0](1/\sqrt{2})$. On the the right we depict $\boldsymbol{x}\bullet\boldsymbol{y}=\boldsymbol{k}_{v_{1}\circ v_{3}}+\boldsymbol{k}_{v_{2}\circ v_{3}}$, where $\circ$ is the group product in $\mathsf{SO}(3)$. The points $v_1$ and $v_2$ are rotated according to $v_3$, which is associated to a rotation matrix of $45^{\circ}$ around the $z$ axis.
}
\label{fig_rkhs_on_sphere}
\end{figure*}

%%--------- End of Figure -----------







We now discuss those RKHS where the domain of the signals is a group, $G$. Although algebraic variants of the group signal processing model are built upon the \textit{group algebra}, $L^{1}(G)$, it is possible to process information on groups with other algebras and arbitrary vector spaces of signals~\cite{lga_icassp,lga_j}. We now proceed to build one of these algebras that is also endowed with the structure of an RKHS.




%%------------------------------------
%%------------ THEOREM ---------------
%%------------------------------------

\begin{corollary}\label{cor_general_A_rkhs_group}
Let $\ccalH\subset\ccalF(\ccalG,\mbF)$ be an RKHS with reproducing kernel $K(u,v)$ and where $\ccalG$ is a group with group product $\circ$ and identity element $1_{\ccalG}$. Let $\ccalA_{\ccalH(K)}$ be the set associated with $\ccalH(K)$ according to~\eqref{eq_A_rkhs_gen} in Theorem~\ref{thm_general_A_rkhs}. Then, $\ccalA_{\ccalH}$ is an associative algebra with product given by~\eqref{eq_A_rkhs_gen_prod} and where 
%
%
%
\begin{equation}
\theta (u,v)
      =
      u\circ v
      ~\text{and}~
      \delta = 1_{\ccalG}
      .
\end{equation}
%
%
%
\end{corollary}

\begin{proof}  See Appendix~\ref{proof_cor_general_A_rkhs_group}  \end{proof}

%%-------- End of Theorem ------------


It is important to remark that the algebra, $\ccalA_{\ccalH}$, introduced in Corollary~\ref{cor_general_A_rkhs_group} relies on the existence of an RKHS structure for a family of functions defined on the group. This is, it is necessary to have a well-defined inner product for the functions defined on the group. 







%%-------------------------------------------------------
%%------------  E X A M P L E  --------------------- 
%%-------------------------------------------------------

\begin{example}\normalfont
\label{ex_rkhs_on_sphere}
%
To clarify the ideas mentioned above about groups and RKHS and to emphasize concrete applications, we focus our attention on functions defined on the sphere $G = \mbS^{n}$. Since $G$ is a Lie group, traditional group signal processing can be used to process signals defined on $G$. However, as we will show next, by choosing the right class of functions $G$, one can define new convolutional signal models based on RKHS algebras. Let us start recalling a few basic facts about RKHS on the sphere following~\cite{cucker2002mathematical}. Let us denote consider functions defined on the $n$-dimensional sphere $\ccalT = \mbS^{n}$. Let $\ccalH_{d} = \ccalH_{d}\left( \ccalT \right)$ be the space of homogeneous polynomials of degree $d$ with independent variables $t_0,t_1, \ldots, t_n$. Any element $\boldsymbol{f}\in\ccalH_d$ can be written as
%
%
$
\boldsymbol{f}
    =
     \sum_{\vert\alpha\vert = d}
          w_{\alpha}
          t^{\alpha}
          ,
$
%
%
where $\alpha = \left( \alpha_0, \alpha_1, \ldots, \alpha_n\right)\in\mbN^{n+1}$ and 
%
%
$
t^{\alpha}
= t_{0}^{\alpha_0}t_{1}^{\alpha_1}\ldots t_{n}^{\alpha_n}
.
$
%
%
As pointed out in~\cite{cucker2002mathematical}, $\ccalH_{d}$ can be endowed with an inner product, $\langle, \rangle_{\ccalH_{d}}$. To see this, let us consider 
%
%
$
\boldsymbol{f}
    =
     \sum_{\vert\alpha\vert = d}
          w_{\alpha}
          t^{\alpha}
$
%
%
and
%
%
$
\boldsymbol{g}
    =
     \sum_{\vert\alpha\vert = d}
          v_{\alpha}
          t^{\alpha}
$
%
%
we have
%
%
%
\begin{equation}\label{eq_inner_prod_Hd}
\left\langle 
     \boldsymbol{f}
     ,
     \boldsymbol{g}
\right\rangle_{\ccalH_{d}}
     =
     \sum_{\vert \alpha\vert =d}
           w_{\alpha}
           v_{\alpha}
               \left( C_{\alpha}^{d}\right)^{-1}
               ,
\end{equation}
%
%
%
where $C_{\alpha}^{d}=d!/(\alpha_{0}!\ldots \alpha_{n}!)$. The kernel, $K: \ccalT\times\ccalT\to\mbR$, associated to $\ccalH_{d}$ as a RKHS is given by
%
%
$
 K(u,v) 
       =
        \langle 
               u, v
        \rangle^{d}   
        ,
$
%
%
where $\langle , \rangle$ is the ordinary inner product in $\mbR^{n+1}$. Then, in the light of Corollary~\ref{cor_general_A_rkhs_group} we have an algebra, $\ccalA_{\ccalH_d}$, that can used to define a convolutional signal processing model associated to $\ccalH_d$ given by $(\ccalA_{\ccalH_d}, \ccalH_d, \rho)$, where $\ccalA_{\ccalH_d}$ is given according to Corollary~\ref{cor_general_A_rkhs_group} and where the homomorphism $\rho: \ccalA_{\ccalH_{d}}\to \ccalB (\ccalH_{d})$ is given by~\eqref{eq_rho_in_rkhs_a} with $\theta (i,j)=i\circ j$, and
%%
%%
%%
%\begin{equation}
%\rho\left( 
%         \sum_{u}\alpha_{u}\boldsymbol{k}_{u}
%    \right)
%    \left\lbrace 
%         \sum_{v}\beta_{v}\boldsymbol{k}_{v}
%    \right\rbrace
%    =
%    \sum_{u,v}\alpha_{u}\beta_{v}\boldsymbol{k}_{u\circ v}
%    ,
%\end{equation}
%%
%%
%%
where $\circ$ is the group operation on $G=\mbS^{n}\subset\mbR^{n+1}$ as a Lie group and $\ccalB (\ccalH_d)$ is the set of bounded operators from $\ccalH_d$ onto itself.
%    
%
\end{example}

%%--------  End of   E X A M P L E   -------------




Example~\ref{ex_rkhs_on_sphere} highlights important implications for performing convolutions with different degrees of complexity on the sphere. This is, we can select the degree of the polynomials that we are going to use as signals and filters and perform convolutions that produce again polynomials of the same degree. Additionally, notice that the function
%
%
$\boldsymbol{k}_{v}(u)
     =  \langle 
               u, v
        \rangle^{d}  
$
%
%
is locally concentrated, i.e. it fades as $x$ and $y$ get away from each other on the sphere and reach exactly zero value when $x$ and $y$ are orthogonal -- see Fig.~\ref{fig_rkhs_on_sphere}. As shown in~\cite{lga_j,lga_icassp} the monomial terms in any element of $\ccalH_d$, dictates specific points on $G = \mbS^{n}$ that uniquely determine bandlimited functions in $L^{1}(G)$. This is, the model $(\ccalA_{\ccalH_d}, \ccalH_d, \rho)$, allows us to perform a $d$-approximated version of the traditional group convolutional signal processing and in the light of the results derived in~\cite{lga_j,lga_icassp}, such results can be uniquely related with more general filters and signals defined on the group. Fig.~\ref{fig_rkhs_on_sphere} displays examples of functions in the RKHS described in Example~\ref{ex_rkhs_on_sphere} and the result of performing a convolution according to the algebra $\ccalA_{\ccalH_{d}}$.

















%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%% SUB - SECTION %%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{RKHS Algebras from Graphons}
\label{sec_gphonsp_rkhs}




%%-----------------------------------
%%------------ FIGURE ---------------
%%-----------------------------------

\begin{figure*}
%
%--------- FIRST ROW ---------
%
\centering
       \begin{subfigure}{.32\linewidth}
	   \centering
          \includegraphics[width=0.8\textwidth]{./figures/graphon_rkhs/fig_6.pdf} 
       \end{subfigure}
    	\begin{subfigure}{.32\linewidth}
		\centering
            \includegraphics[width=1\textwidth]{./figures/graphon_rkhs/fig_5.pdf} 
\end{subfigure}
    	\begin{subfigure}{.32\linewidth}
		\centering
  \includegraphics[width=0.8\textwidth]{./figures/graphon_rkhs/fig_7.pdf} 
\end{subfigure}
%
%
\caption{Depictions of the functions $\boldsymbol{k}_{v}(u)=K(u,v)$ in the RKHS graphon model considering the graphon $W(u,v)=\min(u,v)(1-\max(u,v))$. We show $K(u,v)$ with $u$ ranging from $0$ to $1$ and $v$ ranging from $0$ to $0.5$, $0.8$, and $0.4$. We restrict the values of $v$ to show how the behavior of $\boldsymbol{k}_{v}(u)$ concerning $K(u,v)=W\square W$. The kernel, $K(u,v)$, is determined using the box product between the graphon, $W$, with itself. We depict $\boldsymbol{k}_{0.5}(u)$ (left) and $\boldsymbol{k}_{0.8}(u)$ (left) and the result of their convolution, $\boldsymbol{k}_{0.5}(u)\bullet\boldsymbol{k}_{0.8}(u) = \boldsymbol{k}_{0.5\times 0.8}(u) =\boldsymbol{k}_{0.4}(u)$.}
\label{fig_rkhs_on_graphon}
\end{figure*}

%%--------- End of Figure -----------





Graphons have become a ubiquitous tool for processing information on graphs of large dimension~\cite{gphon_pooling_c,gphon_pooling_j,lovaz2012large}. A graphon is a symmetric bounded measurable function, $W: [0,1]^2 \to [0,1]$, that can be conceived as the limit of an adjacency matrix of a graph whose number of nodes and edges grows up to infinity~\cite{lovaz2012large}. For each graphon, $W(u,v)$, there is one associated integral operator $T_{W}:L^{2}([0,1])\to L^{2}([0,1])$ given by
%
%
%
\begin{equation}\label{eq_T_gphon_shift}
T_{W}\left\lbrace
                  \boldsymbol{x}
              \right\rbrace
      =
      \int_{0}^{1}W(u,v)\boldsymbol{x}(u)du
      .
\end{equation}
%
%
%
The properties of $T_{W}$ can be used to study the properties of $W(u,v)$~\cite{lovaz2012large}. This is done by relating the spectral properties of $T$ with those of $W(u,v)$. More specifically, since $T_{W}$ is compact, normal, and Hilbert-Schmidt with eigenvalues $\lambda_i$ and eigenvectors $\boldsymbol{\varphi}_i$ -- which are orthonormal basis for $L_{2}([0,1])$ -- it can be shown that
%
%
%
\begin{equation}
W(u,v) = \sum_{i=1}^{\infty}
              \lambda_{i}
              \boldsymbol{\varphi}_{i}(u)
              \boldsymbol{\varphi}_{i}(v)
              .
\end{equation}
%
%
%
Additionally, one can leverage $T_{W}$ to define a convolutional signal processing model defined \textit{on} $W(u,v)$~\cite{gphon_pooling_c,gphon_pooling_j}. This can be done with the ASM $(\mbC[t],L_{2}([0,1]),\rho_{W})$, where $\mbC[t]$ is the polynomial algebra with independent variable $t$, $L_{2}([0,1])$ is the set of square integrable functions on $[0,1]$ with the Lebesgue measure, and $\rho_{W}: \mbC[t]\to\ccalB(L_{2}([0,1]))$ is the homomorphism that maps $t$ into $T_{W}$. Then, if $p(t)$ is a polynomial, the action of $\rho_{W}$ can be written as
%
%
%
\begin{equation}
\rho_{W}\left( p(t) \right)
       \left\lbrace 
              \boldsymbol{x}
       \right\rbrace
            =
            p\left(
                 T_{W}
             \right)
                    \left\lbrace 
                             \boldsymbol{x}
                   \right\rbrace
            .
\end{equation}
%
%
%



Now we focus our attention on building an alternative convolutional model on graphons. To do so, we start recalling Theorem~\ref{thm_kernel_from_box_prod} considering as a symbol the graphon $W(u,v)$. Then, we have that given a graphon $W(u,v)$ we can obtain a kernel -- in the sense of Definition~\ref{def_kernel} -- utilizing the box product given by $K(u,v)= (W\square W)(u,v)$, which can be written in terms of the eigenvectors of $W(u,v)$ as we show in the following result. 


%%-----------------------------------
%%----------- LEMMA -----------------
%%-----------------------------------

\begin{corollary}\label{corll_K_from_W}
%
Let $W(u,v)$ be a graphon with eigenvectors $\boldsymbol{\varphi}_{i}(u)$ and eigenvalues $\lambda_i$. Then, the function
%
%
%
\begin{equation}\label{eq_K_from_W}
K(u,v) =
W^{n\square}
=
        \sum_{i=1}^{\infty}
             \lambda_{i}^{n}
             \boldsymbol{\varphi}_{i}(u)
             \boldsymbol{\varphi}_{i}(v)
             ,
\end{equation}
%
%
%
with $n\in\mbN$ and $n\geq 2$, is a kernel in the sense of Definition~\ref{def_kernel}. Additionally, if $K$ is continuous, $K$ is a Mercer kernel. $W^{n\square}$ indicates the $n$-times box product of $W$ with itself.
\end{corollary}

\begin{proof}
    See Appendix~\ref{proof_corll_K_from_W}.
\end{proof}

%%-------- End of Lemma -------------





With Corollary~\ref{corll_K_from_W} at hand we are ready to discuss convolutional graphon signal models relying on $\ccalA_{\ccalH(K)}$ and $\ccalA_{K}$. We start with an example where we show how the traditional graphon signal processing paradigm can be seen under the light of convolutional RKHS models. 






%%---------------------------------------------------------------
%%------------------- E X A M P L E  ----------------------- 
%%---------------------------------------------------------------

\begin{example}\normalfont
\label{ex_gphonsp_rkhs_AK}
%
Let $W$ be a graphon and let $K$ be the kernel given according to~\eqref{eq_K_from_W}. Let $\ccalH(K)$ be the RKHS with reproducing kernel $K$ given according to~\eqref{eq_HK_in_L2_as_rkhs} and let us recall that the classical convolutional signal model on graphons given by  $(\mbC[t],L_{2}([0,1]),\rho_{W})$ where $\rho_{W}$ is a homomorphism with $\rho_{W}(t)=T_{W}$. If we take into account that
%
%
$
T_{W}^{n}\lbrace \boldsymbol{x}\rbrace
=  
T_{K}\lbrace \boldsymbol{x}\rbrace
,
$
%
%
we can see that for any polynomial $p(t)\in\mbC[t]$ we have 
 %
 %
 %
 \begin{equation}\label{eq_ex_gphonsp_rkhs_AK_1}
p\left( 
         T_{W}^{n}
   \right)      
         \lbrace \boldsymbol{x}\rbrace
=  
p\left( 
         T_{K}
   \right)  
          \lbrace \boldsymbol{x}\rbrace
          .
 \end{equation}
%
%
%
Then, since $K$ is a Marcer Kernel, in the light of Theorem~\ref{thm_alg_rkhs_vs_alg_classic} we can see that 
%
%
%
\begin{equation}\label{eq_ex_gphonsp_rkhs_AK_2}
\rho_{W}\left( 
              p\left(
                     t^{n}
                \right)      
       \right)
             \left\lbrace 
                    \boldsymbol{x}
             \right\rbrace
             =
              p\left(
                   \rho_{W}\left( t \right)^{n}
                \right)      
             \left\lbrace 
                    \boldsymbol{x}
             \right\rbrace             
             =
               \rho_{K}
                     \left(
                           p\left( 
                                    K \vert \square
                              \right)
                     \right)
                              \left\lbrace 
                                    \boldsymbol{x}
                             \right\rbrace
                      ,
\end{equation}
%
%
%
for all $\boldsymbol{x}\in\ccalH(K)$.  This is, the RKHS convolutional model $(\ccalA_{K}, \ccalH(K), \rho_{K})$ is compatible with $(\mbC[t],L_{2}([0,1]),\rho_{W})$. Such compatibility, quantified by~\eqref{eq_ex_gphonsp_rkhs_AK_2}, emphasizes that the diffusions in $(\ccalA_{K}, \ccalH(K), \rho_{K})$ are $n$-times higher in order -- the order of the polynomial operator -- with respect to the diffusions in $(\ccalA_{K}, \ccalH(K), \rho_{K})$. This is, the same polynomial expression $p(t)$ leads to diffusions in $(\mbC[t],L_{2}([0,1]),\rho_{W})$ that are of higher order than those in $(\ccalA_{K}, \ccalH(K), \rho_{K})$. Notice that $\ccalH(K)$ is a proper subset of $L_{2}([0,1],\mu)$. This restriction of the class of signals considered comes as the price to pay for having an RKHS structure in $L_{2}([0,1],\mu)$. 
%
\end{example}

%%---------- E N D  of   E x a m p l e  -------------------




One important aspect to remark about Corollary~\ref{corll_K_from_W} is the fact that different choices of $n$ in~\eqref{eq_K_from_W} lead to kernels that capture diffusions -- in the classical Gphon-SP model -- that have different selectivity. This can be observed from the fact that the function $\vert \lambda\vert^{n}$  concentrates around $\vert \lambda\vert =1$ when $[-1,1]$ which is where the spectrum of the graphon $W$ is contained -- see~\cite[p. 124, 131]{lovaz2012large}. This guarantees that the classical diffusions for large values of $n$ are more concentrated around the low frequencies, which by standard convention are associated to those eigenvalues close to $\vert \lambda\vert =1$. This shows that the algebra $\ccalA_{K}$ encapsulates naturally multiresolution attributes in its subsets of filters while allowing us to process signals in subsets of $\subset L_{2}([0,1],\mu)$ while exploiting the attributes of the RKHS $\ccalH(K)$.

Now, we discuss an example of an RKHS convolutional model on graphs where we leverage the algebra $\ccalA_{\ccalH(K)}$.






%%---------------------------------------------------------------
%%------------------- E X A M P L E  ----------------------- 
%%---------------------------------------------------------------

\begin{example}\normalfont
\label{ex_gphonsp_rkhs_AHK}
%
Considering $K$ as in~\eqref{eq_K_from_W} with $n=2$ we have an induced RKHS, $\ccalH (K)$, which defines a subset of functions in $L_{2}([0,1])$ and is given by~\eqref{eq_HK_in_L2_as_rkhs}. We can define a graphon convolutional signal model, $(\ccalA_{\ccalH(K)},\ccalH(K),\rho_{\ccalH(K)})$, where $\ccalA_{\ccalH(K)}$ is the algebra obtained from $\ccalH(K)$ according to Theorem~\ref{thm_general_A_rkhs} with $\theta (u,v) = uv
    ,
    ~\text{and}~
    \delta = 1
    .
$
%
%
with the homomorphism  
%
%
%
\begin{equation}
\rho_{\ccalH(K)}\left( 
                                \sum_{u\in\ccalU}\alpha_{u}\boldsymbol{k}_{u}
                          \right)
    \left\lbrace 
                  \sum_{v\in\ccalV}\beta_{v}\boldsymbol{k}_{v}
    \right\rbrace
    =
    \sum_{u\in\ccalU,v\in\ccalV}\alpha_{u}\beta_{v}\boldsymbol{k}_{uv}
    .
\end{equation}
%
%
%
In Fig.~\ref{fig_rkhs_on_graphon} we depict some of the functions $\boldsymbol{k}_{v}(u)$ in the RKHS graphon model. It is worth pointing out that we could have defined another convolutional model with $\ccalA_{\ccalH(K)}$ by considering $\theta(i,j)=(i+j)\text{mod}[0,1]$, i.e. the sum modulo 1 in the real numbers and choosing $0$ as the unit element of the sum.
%
\end{example}

%%---------- E N D  of   E x a m p l e  -------------------



Although Example~\ref{ex_gphonsp_rkhs_AHK} may seem counter intuitive when compared with the classical Gphon-SP model, it is still a type of convolutional model that can be used to perform scalable filtering and learning while keeping the advantages of working in an RKHS. 
















==> v12/sec_frechet_derivatives.tex <==
%!TEX root =../compiler_paper.tex





%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%% SECTION %%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\section{Fr\'echet Derivatives of Cost Function}






%%----------------------------------
%%--------- THEOREM ----------------
%%----------------------------------

\begin{theorem}\label{thm_Frcht_comp}
Let $\ccalH_1$, $\ccalH_2$ and $\ccalH_3$ be normed vector spaces and let $\ccalU\subset\ccalH_1$ be an open subset of $\ccalH_1$. Let us consider the functions $F_{1}: \ccalH_1 \to \ccalH_2$, $F_2: \ccalH_2 \to \ccalH_3$ and the composition between $F_1$ and $F_2$ represented by $F_{2}\circ F_{1}: \ccalH_1 \to \ccalH_3$. Let $\bbD_{F_1}(u)\{ \cdot \}$ and $\bbD_{F_2}(F_{1}(\boldsymbol{u}))\{ \cdot \}$ be the Fr\'echet derivatives of $F$ and $F_2$ at $u$ and $F_{1}(\boldsymbol{u})$, respectively. Then we have
%
%
%
\begin{equation}
\bbD_{\left(F_{2}\circ F_{1}\right)(\boldsymbol{u})}  \{ \boldsymbol{h} \} 
=
\bbD_{F_{2}}(F_{1}(\boldsymbol{u})) \left\lbrace 
                        \bbD_{F_{1}}(\boldsymbol{u})
                              \{ \boldsymbol{h} \} 
                    \right\rbrace
                    .
\end{equation}
%
%
%
\end{theorem}

\begin{proof}
    See Appendix~\ref{proof_thm_Frcht_comp}.
\end{proof}

%--------- End of Theorem -----------













% %%----------------------------------
% %%--------- THEOREM ----------------
% %%----------------------------------

% \begin{theorem}
% Let $G(\boldsymbol{h}) = \boldsymbol{\alpha}\bullet F(\boldsymbol{h}) + \boldsymbol{\beta}$
% \end{theorem}

% \begin{proof}

% \begin{equation}
% \boldsymbol{\alpha} 
%     \bullet
%         F\left( 
%              \boldsymbol{h}
%              +
%              \boldsymbol{d}
%          \right)
%          -
% \boldsymbol{\alpha} 
%     \bullet         
%         F\left( 
%              \boldsymbol{h}
%          \right)
%          =
% \boldsymbol{\alpha} 
%     \bullet 
%    \bbD_{F}(\boldsymbol{h})
%            \{ \boldsymbol{d} \}
%            +
%            o(\boldsymbol{d})
% \end{equation}
    
% \end{proof}

% %--------- End of Theorem -----------






% %%----------------------------------
% %%--------- THEOREM ----------------
% %%----------------------------------

% \begin{theorem}
% %
% Let $G(\boldsymbol{h}) = \eta\left( \boldsymbol{\alpha}\bullet F(\boldsymbol{h})\right)$. Then, it follows that
% %
% %
% %
% \begin{equation}
% \bbD_{\eta}\left( 
%                  \boldsymbol{\alpha}
%                  \bullet
%                  F\left(\boldsymbol{h}\right)
%            \right)
%            \left\lbrace 
%                  \boldsymbol{\alpha}
%                      \bullet
%                   \bbD_{F}\left( 
%                                \boldsymbol{h}
%                           \right)
%                           \left\lbrace 
%                                \boldsymbol{d}
%                           \right\rbrace
%            \right\rbrace
% \end{equation}
% %
% %
% %   
% \end{theorem}

% %--------- End of Theorem -----------


























%%------------------------------------------
%%------------- PROPOSITION ----------------
%%------------------------------------------

\begin{prop}\label{prop_derivative_nonlin_and_filter}
%
%
Let $\ccalH(K)$ be an RKHS with reproducing kernel $K$. Given a filter $\boldsymbol{h}\in \ccalA_{\ccalH(K)}$ -- see Theorem~\ref{thm_general_A_rkhs} --  and an input signal $\boldsymbol{x}\in \mathcal H(K)$, let $F(\boldsymbol{h}):\mathcal H(K)\to \ccalH(K)$ as
%
%
$
F (\boldsymbol{h})
      =
        \eta\left(  
               \boldsymbol{h}\bullet\boldsymbol{x}
            \right)    
$,
%
%
where $\eta$ is a point-wise non-linearity as specified in Section~\ref{sub_sec_nonlinearity}. Then,
%
%
%
\begin{equation}
   \bbD_{F}(\boldsymbol{h})
         \left\lbrace 
               \boldsymbol{d}
         \right\rbrace
         =
         \bbD_{\eta}\left( 
                       \boldsymbol{h}\bullet\boldsymbol{x}
                    \right)
                          \left\lbrace 
                               \boldsymbol{d}
                               \bullet
                               \boldsymbol{x}
                          \right\rbrace
                          .
\end{equation}
%
%
%
\end{prop}

\begin{proof}
    See Appendix~\ref{proof_prop_derivative_nonlin_and_filter}.
\end{proof}


%%---------- End of Proposition ------------














% %%---------------------------------------
% %%------------- THEOREM -----------------
% %%---------------------------------------

% \begin{theorem}
% \label{thm_one_layer_derivative}
% %
% Let $\ccalH(K)$ be an RKHS with reproducing kernel $K$. Then, given a reference signal $\boldsymbol{r}\in \ccalH(K)$, a convolutional filter $\boldsymbol{h}\in \mathcal \ccalA_{\ccalH(K)}$ -- see Theorem~\ref{thm_general_A_rkhs} --  and an input signal $\boldsymbol{x}\in \mathcal H(K)$,  define $\ell(\boldsymbol{h}):\ccalH(K)\to \mathbb R$ as the quadratic error between the reference and the output signal $\boldsymbol{y}=\eta(\boldsymbol{h}\bullet \boldsymbol{x})$ as a function of the filter, i.e.,  
% %
% %
% $
% \ell(\boldsymbol{h})
%         =
%          \frac{1}{2}
%             \left\Vert
%                   \boldsymbol{r}
%                   -
%                   \eta\left(
%                          \boldsymbol{h}\bullet \boldsymbol{x}
%                       \right)
%             \right\Vert_{\calH(K)}^2
%             ,
% $
% %
% %
% where $\eta$ is the point-wise nonlinearity. Then 
% %
% %
% %
% \begin{multline}
% \bbD_{\ell(\boldsymbol{h})}(\boldsymbol{h})
%     \left\lbrace
%         \boldsymbol{d}
%     \right\rbrace 
%   =
%   \\
%   -
%   \left\langle 
%        \bbD_{\eta}(\boldsymbol{h}\bullet\boldsymbol{x})
%                \left\lbrace 
%                      \boldsymbol{d}\bullet\boldsymbol{x}
%                \right\rbrace
%        ,
%        \boldsymbol{r}
%        -
%        \eta\left( \boldsymbol{h}
%                         \bullet
%                   \boldsymbol{x}
%             \right)
%   \right\rangle_{\ccalH(K)}
%   .
% \end{multline}
% %
% %
% %
% \end{theorem}

% \begin{proof}
% See Appendix~\ref{proof_thm_one_layer_derivative}.
% \end{proof}
% %%---------- End of Theorem -------------
















































% %%---------------------------------------
% %%------------ COROLLARY ----------------
% %%---------------------------------------

% \begin{corollary}
% If we consider Proposition~\ref{prop:derivative_loss_conv} with the product $\bullet$ given by the ordinary convolution in $L^{1}(\mbR)$, $\ast$, then we have 
% %
% %
% %
% \begin{multline}
% \bbD_{\ell(h)}(h) \{ \xi \} 
%     =
%     \\
%      \sum_{u,v,\ell}
%             \bbx(u)
%             \bbx(v)
%             \bbh(\ell)
%                 \left( 
%                      \boldsymbol{k}_{u}\ast \xi
%                 \right)(v+\ell)
%       -
%       \sum_{u,\omega}
%             \bbx(u)
%             \bbr(\omega)
%                  \left( 
%                        \boldsymbol{k}_{u}\ast \xi
%                  \right)(\omega)
% \end{multline}
% %
% %
% %
    
% \end{corollary}

% %%-------- End of Corollary -------------









% Inspecting \eqref{eq:derivative_convolution} we observe   

% \begin{align} &x(-t)*(h*x-r)\\
% &=\sum_i X_i k(t_i,-t)*\left(\sum_j H_j k(t_j,t)* \sum_n X_n k(t_n,t)\right)\\
% &-\sum_i X_i k(t_i,-t)*\left(\sum_j R_j k(t_j,t)\right)\\
% &=\sum_i \sum_j \sum_n X_i H_j X_n k(-t_i,t)* k(t_j,t)*k(t_n,t)\\
% &-\sum_i\sum_j X_i R_j  k(-t_i,t)* k(t_j,t)\\
% &=\sum_i \sum_j \sum_n X_i H_j X_n  k(t_n+t_j-t_i,t)\label{eq:derivative_convolution_xhx}\\
% &-\sum_i\sum_j X_i R_j  k(t_j-t_i,t)
% \label{eq:derivative_convolution_rx}
% \end{align}


% \textbf{\textcolor{blue}{Remark}}
% Training a convolutional system consisting on a single filter and a quadratic loss via stochastic gradient descent involves incorporating  \eqref{eq:derivative_convolution}  to the filter sequentially.

% Notice that according to \eqref{eq:derivative_convolution_rx}, if the input has a kernel at  $t_i$ and the reference has a kernel at $t_j$, then the filter has a kernel at $t_j-t_i$, so that next inputs will be translated this  distance between input and output reference  $t_j-t_i$ seen during training. 

% \juan{I tried to take derivatives with respect to the non-linearity on the coefficients below. Not exactly, I got the differential instead.}
% \juan{ An alternative would be to take the linearity with respect to  the signal itself.  But then the signal does not belong to $\calH$ anymore.  Think of  expressing this nonlinearity in terms of samples of the signal, and go from the coefficients to these samples multiplying by the matix of kernels. Then we could apply Proposition 2 (the Frechet derivative of the evaluation operational. But not really, since Proposition 2 is for a constant point $t_0$ that does not depend on the signal, so using its knots is not correct. }







% \subsection{Differential of $\sigma(z)$}
% \begin{prop}\label{prop:derivative_relu}
% Consider the RELU nonlinearity defined as $\sigma:\mathcal H\to\mathcal H$ such that \begin{align}
%     \sigma\left(\sum_i Z_i k(t_i,t)\right)=\sum_i \max\{0,Z_i\} k(t_i,t)
% \end{align}

%  Then the differential of $\sigma(z)$ is given by 

%  \begin{align}
%  d\sigma=\sigma(dz)    
%  \end{align}
%  \juan{The following proof assumes that the knots of $z$ and $dz$ do not coincide. It should be easy to proof otherwise.}
%  \end{prop}
% \begin{proof}
% If $z(t)=\sum_i Z_i k(t_i,t)$ and $dz(t)=\sum_j dZ_j k(t_j,t)$ 
% \begin{align}
%     &\sigma(z+dz)-\sigma(z)-\sigma(dz)=\sum_i \max\{0,Z_i\}k(t_i,t)\\&+\sum_j \max\{0,dZ_j\}k(t_j,t)-\sum_i \max\{0,Z_i\}k(t_i,t)\\
%     &-\sum_j \max\{0,dZ_j\}k(t_j,t) \\&=0
% \end{align}
    
% \end{proof}
 


% \subsection{Differential of $l(h)=\frac{1}{2}\|r-\sigma(h*x)\|^2$}
% \begin{prop}\label{prop:derivative_relu}

%  Then the differential of $l(h)$ is given by 

%  \begin{align}
%  dl=<y-r,\sigma(x*dh)>    
%  \end{align}
%  \end{prop}
% \begin{proof}
% Substitute $dz=x*dh$ and $dy=\sigma(dz)$ in $dl=<dy,y-r>$ according to \eqref{eq:derivative_loss}
    
% \end{proof}

% Next, we need to find $\tilde h$ such that $dl=<y-r,\sigma(x*\tilde h)> $ is positive, in order to build gradient descent algorithm as

% \begin{align}
%     h_{k+1}=h_k-\eta \tilde h
% \end{align}

% For this purpose we  write

% \begin{align}
% &dl=<y-r,\sigma(x*\tilde h)> \\
% &=\left\langle \sum_iY_ik(t_i,t)-\sum_jR_jk(t_j,t), \sum_{m,n} \sigma(\tilde H_m,X_n) k(t_{m}+t_n,t) \right\rangle\\
% &=    \sum_i \sum_{m}\sum_nY_i \max\{0,\tilde H_mX_n\}k(t_m+t_n,t_i) \\
% &-    \sum_j \sum_{m} \sum_{n}R_j \max\{0,\tilde H_mX_n\}k(t_m+t_n,t_j) \\
% &=     \sum_i \sum_m \sum_n  Y_i \max\{0,\tilde H_mX_n\}k(t_m,t_i-t_n) \\
% &-    \sum_j  \sum_{n}\sum_{m} R_j  \max\{0,\tilde H_mX_n\}k(t_m,t_j-t_n)  
% \end{align}
% \juan{Need to find $\tilde H_m$ and $t_m$ such that this expression is positive }



%\juan{We want 
%
%\begin{align}
%I&=<r-F(h),D_F(h)\{d\}>0\\
%D_F(h)\{d\}&=r-F(h)\\
%A&=<r-F(h),r-F(h)>0\\
%U&=<r-F(h),r-F(h)-D_F(h)\{d\}>\\
%U&=<r-F(h),S>\\
%I&=A-U>0 \iff U<A
%\end{align}
%}




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%% Sub - SECTION %%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Proof of Theorem~\ref{thm_F1_F2_derivatives}}
\label{proof_thm_F1_F2_derivatives}

\begin{proof}

First, we start considering the functions
%
%
%
\begin{equation}
G_{1} (\boldsymbol{h})
     = 
     \eta\left(
              \boldsymbol{h}\bullet\boldsymbol{\alpha}
         \right)
         ,
\end{equation}
%
%
%
and
%
%
%
\begin{equation}
G_{2} (\boldsymbol{h})
     = 
     \sum_{i=1}^{N_2}
          \eta 
             \left(                  
                  \boldsymbol{\beta}_i
                    \bullet
                  \boldsymbol{h}
                  +
                  \boldsymbol{\gamma}_i
             \right)
             .
\end{equation}
%
%
%

Then, we take into account that $F^{(1)}(\boldsymbol{h}) = \left( G_{2}\circ G_1 \right) (\boldsymbol{h})$. If we apply the chain rule for the Fr\'echet derivative of
$\left( G_{2}\circ G_1 \right) (\boldsymbol{h})$ it follows that
%
%
%
\begin{equation}
\bbD_{\left(G_2 \circ G_1 \right)}(\boldsymbol{h})\{ \boldsymbol{d} \} 
=
\bbD_{G_2}\left(
               G_1 (\boldsymbol{h})
           \right) 
\left\lbrace 
                \bbD_{G_1}(\boldsymbol{h})\{ \boldsymbol{d} \} 
                    \right\rbrace
\end{equation}
%
%
%
where we know that
%
%
%
\begin{equation}
   \bbD_{G_1}(\boldsymbol{h})
         \left\lbrace 
               \boldsymbol{d}
         \right\rbrace
         =
         \bbD_{\eta}\left( 
                       \boldsymbol{h}\bullet\boldsymbol{\alpha}
                    \right)
                          \left\lbrace 
                               \boldsymbol{d}
                               \bullet
                               \boldsymbol{\alpha}
                          \right\rbrace
                          ,
\end{equation}
%
%
%
and
%
%
%
\begin{equation}
 \bbD_{G_2}(\boldsymbol{h})
      \{ \boldsymbol{d} \}
      =
      \sum_{i=1}^{N_2}
            \bbD_{\eta}
                 \left( 
                     \boldsymbol{\beta}_i 
                        \bullet
                      \boldsymbol{h}
                      +
                      \boldsymbol{\gamma}_i
                 \right)
                    \left\lbrace 
                        \boldsymbol{\beta}_i 
                          \bullet
                        \boldsymbol{d}
                    \right\rbrace
                    .
\end{equation}
%
%
%
Therefore,
%
%
%
\begin{multline}
\bbD_{F^{(1)}}(\boldsymbol{h})\{ \boldsymbol{d} \}
     =
     \\
      \sum_{i=1}^{N_2}
            \bbD_{\eta}
                 \left( 
                     \boldsymbol{\beta}_i 
                        \bullet
                      \boldsymbol{h}
                      +
                      \boldsymbol{\gamma}_i
                 \right)
                    \left\lbrace 
                        \boldsymbol{\beta}_i 
                          \bullet
                                 \bbD_{\eta}\left( 
                       \boldsymbol{h}\bullet\boldsymbol{\alpha}
                    \right)
                          \left\lbrace 
                               \boldsymbol{d}
                               \bullet
                               \boldsymbol{\alpha}
                          \right\rbrace
                    \right\rbrace
                    .
\end{multline}
%
%
%


Now, we evaluate the expressions above for $\boldsymbol{h}=\boldsymbol{h}_{j}^{(1,0)}$, i.e.
%
%
%
$
F\left(
    \boldsymbol{h}_{j}^{(1,0)}
  \right)
     =
      \left(
       G_{2} \circ G_{1}
      \right)\left( 
                \boldsymbol{h}_{j}^{(1,0)} 
             \right)
             ,
$
%
%
%
which leads to
%
%
%
% \begin{multline}
% \bbD_{F^{(1)}}(\boldsymbol{h})\{ \boldsymbol{d} \}
%      =
%      \\
%       \sum_{i=1}^{N_2}
%             \bbD_{\eta}
%                  \left( 
%                      \boldsymbol{h}_{j}^{(2,i)}
%                         \bullet
%                       \boldsymbol{h}
%                       +
%                       \sum_{k\neq j}
%                            \boldsymbol{h}_{k}^{(2,i)}
%                            \bullet
%                            \eta\left( 
%                                   \boldsymbol{h}_{k}^{(1,0)}
%                                     \bullet
%                                   \boldsymbol{x}
%                                \right)
%                  \right)
%                  \\
%                     \left\lbrace 
%                         \boldsymbol{h}_{j}^{(2,i)} 
%                           \bullet
%                                  \bbD_{\eta}\left( 
%                        \boldsymbol{h}
%                             \bullet
%                         \boldsymbol{x}
%                     \right)
%                           \left\lbrace 
%                                \boldsymbol{d}
%                                \bullet
%                                \boldsymbol{x}
%                           \right\rbrace
%                     \right\rbrace
% \end{multline}
% %
% %
% %



%
%
%
\begin{multline}
\bbD_{F}\left(
         \boldsymbol{h}_{j}^{(1,0)}
      \right)
     \left\lbrace 
          \boldsymbol{d}_{j}^{(1,0)}
     \right\rbrace 
     =
     \\
      \sum_{i=1}^{N_2}
            \bbD_{\eta}
                 \left( 
                     \boldsymbol{h}_{j}^{(2,i)}
                        \bullet
                      \boldsymbol{h}
                      +
                      \sum_{k\neq j}
                           \boldsymbol{h}_{k}^{(2,i)}
                           \bullet
                           \eta\left( 
                                  \boldsymbol{h}_{k}^{(1,0)}
                                    \bullet
                                  \boldsymbol{x}
                               \right)
                 \right)
                 \\
                    \left\lbrace 
                        \boldsymbol{h}_{j}^{(2,i)} 
                          \bullet
                                 \bbD_{\eta}\left( 
                       \boldsymbol{h}_{j}^{(1,0)}
                            \bullet
                        \boldsymbol{x}
                    \right)
                          \left\lbrace 
                               \boldsymbol{d}_{j}^{(1,0)}
                               \bullet
                               \boldsymbol{x}
                          \right\rbrace
                    \right\rbrace
\end{multline}
%
%
%

Now, we turn our attention to the Fr\'echet derivative of $F^{(2)}$. We start taking into account that
%
%
$
F^{(2)}(\boldsymbol{h})
 =
  \left(
     G_{2} \circ G_{1}
  \right)(\boldsymbol{h}) 
$
%
%
where
%
%
%
\begin{equation}
G_{1} (\boldsymbol{h})
     = 
     \boldsymbol{h}
        \bullet
      \boldsymbol{\alpha}
      +
      \boldsymbol{\beta}_{i,j}
      ,
\end{equation}
%
%
%
and
%
%
%
\begin{equation}
G_{2} (\boldsymbol{h})
     = 
         \eta\left( 
               \boldsymbol{h}
              \right)
         +
         \boldsymbol{\gamma}_{i,j}
         .
\end{equation}
%
%
%

If we take into account the chain rule property of the Fr\'echet derivative, it follows that
%
%
%
\begin{equation}
\bbD_{\left( G_2 \circ G_1 \right)}(\boldsymbol{h})\{ \boldsymbol{d} \} 
=
\bbD_{G_2}\left(
               G_1 (\boldsymbol{h})
           \right) 
\left\lbrace 
                \bbD_{G_1}(\boldsymbol{h})\{ \boldsymbol{d} \} 
                    \right\rbrace
                    ,
\end{equation}
%
%
%
where
%
%
%
\begin{equation}
\bbD_{G_1}(\boldsymbol{h})
    \left\lbrace 
        \boldsymbol{d}
    \right\rbrace
    =
    \boldsymbol{d}
       \bullet
    \boldsymbol{\alpha} 
    ,
\end{equation}
%
%
%
and 
%
%
%
\begin{equation}
\bbD_{G_2}(\boldsymbol{h})
    \left\lbrace 
        \boldsymbol{d}
    \right\rbrace
    =
    \bbD_{\eta}(\boldsymbol{h})
      \left\lbrace 
          \boldsymbol{d}
      \right\rbrace
      .
\end{equation}
%
%
%
Therefore, 
%
%
%
\begin{equation}
\bbD_{\left( G_2 \circ G_1 \right)}(\boldsymbol{h})
    \left\lbrace 
        \boldsymbol{d}
    \right\rbrace
    =
    \bbD_{\eta}\left(
                    \boldsymbol{h}
                       \bullet
                    \boldsymbol{\alpha}
                    +
                    \boldsymbol{\beta}_{i,j}
                \right)
      \left\lbrace 
          \boldsymbol{d}
              \bullet
          \boldsymbol{\alpha}    
      \right\rbrace
      .
\end{equation}
%
%
%

Then, evaluating the expressions above in $\boldsymbol{h}=\boldsymbol{h}_{j}^{(2,i)}$, it follows that
%
%
%
\begin{multline}
\bbD_{F^{(2)}}
          \left(
               \boldsymbol{h}_{j}^{(2,i)}
          \right)
    \left\lbrace 
        \boldsymbol{d}_{j}^{(2,i)}
    \right\rbrace
    =
    \\
    \bbD_{\eta}\left(
                    \boldsymbol{h}_{j}^{(2,i)}
                       \bullet
                    \eta\left(
                           \boldsymbol{h}_{j}^{(1,0)}
                              \bullet
                           \boldsymbol{x}   
                        \right)
                    +
                    \sum_{k\neq j}
                        \boldsymbol{h}_{k}^{(2,i)}
                             \bullet
                        \eta\left( 
                                \boldsymbol{h}_{j}^{(1,0)}
                                   \bullet
                                \boldsymbol{x}   
                            \right)
                \right)
                \\
      \left\lbrace 
          \boldsymbol{d}_{j}^{(2,i)}
              \bullet
          \eta\left( 
                   \boldsymbol{h}_{j}^{(1,0)}
                      \bullet
                   \boldsymbol{x}   
              \right)
      \right\rbrace
\end{multline}
%
%
%



\end{proof}












%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%% SUB - SECTION %%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Proof of Theorem~\ref{thm_frechet_nonlinearity}}
\label{proof_thm_frechet_nonlinearity}

\begin{proof}

We start by leveraging the definition of the Fr\'echet derivative of $\eta$. 
%
%
%
\begin{multline}
\eta\left( 
         \boldsymbol{h}
         +
         \boldsymbol{d}
    \right)
    -
\eta\left( 
         \boldsymbol{h}
    \right)   
    =
    \\
 \eta\left( 
         \sum_{u\in\ccalU_1}\bbh(u)\boldsymbol{k}_{u}
         +
         \sum_{u\in\ccalU_2}\bbd(u)\boldsymbol{k}_{u}
    \right)   
    -
\eta\left( 
         \sum_{u\in\ccalU_1}\bbh(u)\boldsymbol{k}_{u}
    \right) 
    .
\end{multline}
%
%
%
Now, we take into account that if $\ccalU = \ccalU_1 \bigcup \ccalU_2$ we can write
%
%
%
\begin{equation}
 \boldsymbol{h}=\sum_{u\in\ccalU}\widetilde{\bbh}(u)\boldsymbol{k}_{u}
 ,
 \quad
 \boldsymbol{d}=\sum_{u\in\ccalU}\widetilde{\bbd}(u)\boldsymbol{k}_{u}
\end{equation}
%
%
%
where 
%
%
%
\begin{equation}
\widetilde{\bbh}(u)=
\left\lbrace 
     \begin{array}{ccc}
         \bbh(u)  &  \text{if} & u\in\ccalU_{1} \\
         0 &     \text{otherwise} & 
     \end{array}
\right.
,
\end{equation}
%
%
%
and
%
%
%
\begin{equation}
\widetilde{\bbd}(u)=
\left\lbrace 
     \begin{array}{ccc}
         \bbd(u)  &  \text{if} & u\in\ccalU_{2} \\
         0 &     \text{otherwise} & 
     \end{array}
\right.
.
\end{equation}
%
%
%

Applying the action of $\eta$ in terms of $\widehat{\eta}$ -- see~\eqref{eq_nonlinearity_a} and~\eqref{eq_nonlinearity_b} -- we obtain
%
%
%
\begin{multline}
\eta\left( 
         \boldsymbol{h}
         +
         \boldsymbol{d}
    \right)
    -
\eta\left( 
         \boldsymbol{h}
    \right)   
    =
    \\
    \sum_{u\in\ccalU}\widehat{\eta}_{u}
                \left(
                      \boldsymbol{h}
                      +
                      \boldsymbol{d}
                 \right)
                       \boldsymbol{k}_{u}
    -
    \sum_{u\in\ccalU}
          \widehat{\eta}_{u}
          \left(
              \boldsymbol{h}
          \right)
          \boldsymbol{k}_{u}
          .
\end{multline}
%
%
%
Factoring out the term $\boldsymbol{k}_{u}$ in the sum we obtain
%
%
%
\begin{equation}
\eta\left( 
         \boldsymbol{h}
         +
         \boldsymbol{d}
    \right)
    -
\eta\left( 
         \boldsymbol{h}
    \right)   
    =
         \sum_{u\in\ccalU}
         \left(
         \widehat{\eta}_{u}\left(
                      \boldsymbol{h}
                      +
                      \boldsymbol{d}
                 \right)
    -
          \widehat{\eta}_{u}
          \left(
              \boldsymbol{h}
          \right)
          \right)
          \boldsymbol{k}_{u}
          ,
\end{equation}
%
%
%
which implies
%
%
%
\begin{equation}
 \bbD_{\eta}(\boldsymbol{h})
          \left\lbrace 
                 \boldsymbol{d}
          \right\rbrace 
          =
          \sum_{u\in\ccalU}
                      \bbD_{\widehat{\eta}_{u}}
                           \left(
                               \boldsymbol{h}
                           \right)
                           \left\lbrace 
                                  \boldsymbol{d}
                           \right\rbrace
                 \boldsymbol{k}_{u}
                 .
\end{equation}
%
%
%    

Now, we calculate the explicit expression for
%
%
$ \bbD_{\widehat{\eta}_{u}}
                           \left(
                               \boldsymbol{h}
                           \right)
                           \left\lbrace 
                                  \boldsymbol{d}
                           \right\rbrace
                           .
$
%
%
We proceed taking into account that
%
%
%
\begin{equation}
\widehat{\eta}_{u}\left( 
         \boldsymbol{h}
         +
         \boldsymbol{d}
    \right)
    -
\widehat{\eta}_{u}\left( 
         \boldsymbol{h}
    \right)   
    =
    \frac{
       \sigma\left( \boldsymbol{h}(u)+ \boldsymbol{d}(u)\right)
      }
      {
      \sum_{r,u\in\ccalU}\boldsymbol{k}_{u}(r)
      }
      -
      \frac{
       \sigma\left(\boldsymbol{h}(u)\right)
      }
      {
      \sum_{r,u\in\ccalU}\boldsymbol{k}_{u}(r)
      }
          .
\end{equation}
%
%
%
Then, we have
%
%
%
\begin{equation}
\widehat{\eta}_{u}\left( 
         \boldsymbol{h}
         +
         \boldsymbol{d}
    \right)
    -
\widehat{\eta}_{u}\left( 
         \boldsymbol{h}
    \right) 
    =
    \frac{
    \sigma^{'}\left(
                  \boldsymbol{h}(u)
              \right)
              \boldsymbol{d}(u)
    }
    {
     \sum_{r,u\in\ccalU}\boldsymbol{k}_{u}(r)
    }
    =
                          \bbD_{\widehat{\eta}_{u}}
                           \left(
                               \boldsymbol{h}
                           \right)
                           \left\lbrace 
                                  \boldsymbol{d}
                           \right\rbrace
                           .
\end{equation}
%
%
%
With this expression at hand, we finally have 
%
%
%
\begin{equation}
 \bbD_{\eta}(\boldsymbol{h})
          \left\lbrace 
                 \boldsymbol{d}
          \right\rbrace 
          =
          \sum_{u\in\ccalU}
                     \frac{
    \sigma^{'}\left(
                  \boldsymbol{h}(u)
              \right)
              \boldsymbol{d}(u)
    }
    {
     \sum_{r,u\in\ccalU}\boldsymbol{k}_{u}(r)
    }
                 \boldsymbol{k}_{u}     
          ,
\end{equation}
%
%
%
where $\sigma^{'}(\cdot)$ is the ordinary derivative of $\sigma(x)=\max\{ 0,x \}$.




\end{proof}










	
	

% %%------------------------------------------
% %%------------- PROPOSITION ----------------
% %%------------------------------------------

% \begin{prop}\label{prop_derivative_loss_conv}
% %
% Let $\ccalH(K)$ be an RKHS with reproducing kernel $K$. Given a reference signal $\boldsymbol{r}\in \mathcal H(K)$, a filter $\boldsymbol{h}\in \ccalA_{\ccalH(K)}$ -- see Theorem~\ref{thm_general_A_rkhs} --  and an input signal $\boldsymbol{x}\in \mathcal H(K)$,  define $\ell(\boldsymbol{h}):\mathcal H(K)\to \mathbb R$ as the quadratic error between the reference and the output signal $\boldsymbol{y}=\boldsymbol{h}\bullet \boldsymbol{x}$ as a function of the filter, i.e.,
% %
% %
% $
% \ell(
%     \boldsymbol{h}
%     )
%     =\frac{1}{2}
%          \left\Vert 
%                \boldsymbol{r}
%                -
%                \boldsymbol{h}\bullet \boldsymbol{x}
%          \right\Vert_{\calH}^2
% .
% $
% %
% %
% Then,
% %
% %
% %
% \begin{equation}
% \bbD_{\ell(\boldsymbol{h})}(\boldsymbol{h}) 
%        \left\lbrace
%            \boldsymbol{d}
%        \right\rbrace 
%   =
%   \left\langle 
%        \boldsymbol{d}\bullet \boldsymbol{x}
%        ,
%        \boldsymbol{h}\bullet \boldsymbol{x}
%          - 
%         \boldsymbol{r}
%   \right\rangle_{\ccalH(K)}
% \end{equation}
% %
% %
% %
% \end{prop}

% \begin{proof}
%     See Appendix~\ref{proof_prop_derivative_loss_conv}
% \end{proof}

% %%---------- End of Proposition ------------






% %%------------------------------
% %%-------- PROPOSITION ---------
% %%------------------------------

% \begin{prop}
% Given a reference signal $r\in \mathcal H$, define $\ell(y):\mathcal H\to \mathbb R$ such that $\ell(y)=\frac{1}{2}\|r-y\|_{\ccalH}^2$. Then 
% %
% %
% %
% \begin{align}
% \frac{dl}{dy} &= y-r.\label{eq:derivative_loss}
% \end{align}
% %
% %
% %
% \end{prop}

% %%---- End of Proposition ------


% \begin{proof}

% First, let us start taking into account that
% %
% %
% %
% \begin{equation}
% \ell (y)
%  =
%  \frac{1}{2}
%    \left\Vert
%      r
%      -
%      y
%    \right\Vert^2
%    =
%    \frac{1}{2}
%    \left[
%      \Vert r \Vert^2
%      -
%      2
%      \langle
%          r,y
%      \rangle
%      +
%      \Vert
%        y
%      \Vert^2  
%    \right] 
%    ,
% \end{equation}	
% %
% %
% %	
% where $r$ is a fixed function. In order to obtain the Fr\'echet derivative of $\ell (y)$ we compute 
% %
% %
% %
% \begin{multline}
% \ell\left( 
%         y
%         +
%         \xi
%     \right)
%     -
% \ell(y)
%     =
%     \frac{1}{2}
%          \left\Vert
%             y+\xi
%          \right\Vert^2
%     -
%     \frac{1}{2}
%     \left\Vert
%        y
%     \right\Vert^2  
%     -
%     \left\langle
%      r , \xi
%     \right\rangle 
%     \\
%     =
%      -
%           \left\langle
%                \xi 
%                ,
%                r
%           \right\rangle 
%       +
%       \left\langle
%             \xi
%             ,
%              y
%       \right\rangle 
%       +
%       \frac{1}{2}
%       \left\Vert
%            \xi
%       \right\Vert^{2} 
%       .      
% \end{multline}
% %
% %
% %
% then, if we compare with the definition of the Fr\'echet derivative we have
% %
% %
% %
% \begin{equation}
% \bbD_{\ell(y)}(y)\{ \xi \}
%       =   
%            -
%       \left\langle
%         \xi  
%         ,
%         r
%       \right\rangle 
%       +
%       \left\langle
%       \xi
%       ,
%       y
%       \right\rangle 
%       =
%       \left\langle
%            \xi
%            ,
%            y-r
%       \right\rangle
% \end{equation}

% \end{proof}
  





%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%% Sub - SECTION %%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Proof of Proposition~\ref{prop_derivative_loss_Fh}}
\label{proof_prop_derivative_loss_Fh}

\begin{proof}

First, we start taking into account that
%
%
%
\begin{equation}
\ell\left( 
         \boldsymbol{h}  
    \right)
    =
    \frac{1}{2}
    \left[
         \Vert \boldsymbol{r} \Vert^{2}_{\ccalH(K)}
         -
         2\langle \boldsymbol{r}, F(\boldsymbol{h})\rangle_{\ccalH(K)}
         +
         \Vert F(\boldsymbol{h}) \Vert_{\ccalH(K)}^{2}
    \right]
    .
\end{equation}
%
%
%
Then, it follows that
%
%
%
\begin{multline}
\ell\left( 
        \boldsymbol{h}
        +
        \boldsymbol{d}
    \right)    
-
\ell\left(
         \boldsymbol{h}
    \right)
    =
    -\left\langle
           \boldsymbol{r}
           ,
           F\left(
                \boldsymbol{h}
                +
                \boldsymbol{d}
            \right)
            -
            F\left(
                \boldsymbol{h}
            \right)
     \right\rangle_{\ccalH(K)}
     +
     \\
     \frac{1}{2}
            \left[
                  \left\langle 
                        F\left(
                             \boldsymbol{h}
                             +
                             \boldsymbol{d}
                         \right)
                         ,
                         F\left(
                             \boldsymbol{h}
                             +
                             \boldsymbol{d}
                         \right)
                  \right\rangle_{\ccalH(K)}
                  -
                  \left\langle 
                        F\left(
                             \boldsymbol{h}
                         \right)
                         ,
                         F\left(
                             \boldsymbol{h}
                         \right)
                  \right\rangle_{\ccalH(K)}
            \right]
            .
\end{multline}
%
%
%





%
%
%
\begin{multline}
\ell\left( 
        \boldsymbol{h}
        +
        \boldsymbol{d}
    \right)    
-
\ell\left(
         \boldsymbol{h}
    \right)
    =
    \\
    \left\langle 
           F(\boldsymbol{h}+\boldsymbol{d})
            -
           F(\boldsymbol{h})
          ,      
          \frac{1}{2}
                \left[
                      F(\boldsymbol{h}+\boldsymbol{d})
                      +
                      F(\boldsymbol{h})
                \right]
                -
                \boldsymbol{r}
    \right\rangle_{\ccalH(K)}
    .
\end{multline}
%
%
%
Now, taking into account the definition of the Fr\'echet derivative of $F$ it follows that
%
%
%
\begin{multline*}
\ell\left( 
        \boldsymbol{h}
        +
        \boldsymbol{d}
    \right)    
-
\ell\left(
         \boldsymbol{h}
    \right)
    =
    \\
    \left\langle 
           \bbD_{F}(\boldsymbol{h})\left\lbrace 
                                        \boldsymbol{d} 
                                   \right\rbrace
            +
            o\left( \boldsymbol{d} \right)
           ,  
           F(\boldsymbol{h})
           +
          \frac{1}{2}
                \bbD_{F}(\boldsymbol{h})
                    \left\lbrace
                         \boldsymbol{d}
                    \right\rbrace
                -
                \boldsymbol{r}
                +
                 o\left( \boldsymbol{d} \right)
    \right\rangle_{\ccalH(K)}
    .
\end{multline*}
%
%
%
Now, we group and rearrange terms again to obtain
%
%
%
\begin{multline}
\ell\left( 
        \boldsymbol{h}
        +
        \boldsymbol{d}
    \right)    
-
\ell\left(
         \boldsymbol{h}
    \right)
    =
    \left\langle 
           \bbD_{F}(\boldsymbol{h})\left\lbrace 
                                        \boldsymbol{d} 
                                   \right\rbrace
           ,  
           F(\boldsymbol{h})
                -
                \boldsymbol{r}
    \right\rangle_{\ccalH(K)}
    +
    \\
     \left\langle 
           \bbD_{F}(\boldsymbol{h})\left\lbrace 
                                        \boldsymbol{d} 
                                   \right\rbrace
           ,  
          \frac{1}{2}
                \bbD_{F}(\boldsymbol{h})
                    \left\lbrace
                         \boldsymbol{d}
                    \right\rbrace
    \right\rangle_{\ccalH(K)}
    \\
    +
     \left\langle 
           o\left( \boldsymbol{h} \right)
           ,  
                     F(\boldsymbol{h})
           +
          \frac{1}{2}
                \bbD_{F}(\boldsymbol{h})
                    \left\lbrace
                         \boldsymbol{d}
                    \right\rbrace
                -
                \boldsymbol{r}
                +
                 o\left( \boldsymbol{d} \right)
    \right\rangle_{\ccalH(K)}
    .
\end{multline}
%
%
%
Then, taking into account the definition of the Fr\'echet derivative, the fact that $o(\boldsymbol{h})\to 0$ and that the term 
%
%
$
     \left\langle 
           \bbD_{F}(\boldsymbol{h})\left\lbrace 
                                        \boldsymbol{d} 
                                   \right\rbrace
           ,  
          \frac{1}{2}
                \bbD_{F}(\boldsymbol{h})
                    \left\lbrace
                         \boldsymbol{d}
                    \right\rbrace
    \right\rangle_{\ccalH(K)}
$
%
%
is quadratic with respect to $\boldsymbol{d}$ we have that
%
%
%
\begin{equation}
\bbD_{\ell}(\boldsymbol{h})
     \left\lbrace 
           \boldsymbol{d}
     \right\rbrace
     =
     -
     \left\langle 
           \bbD_{F}(\boldsymbol{h})\left\lbrace 
                                        \boldsymbol{d} 
                                   \right\rbrace
           ,  
           \boldsymbol{r}
           -
           F(\boldsymbol{h})
    \right\rangle_{\ccalH(K)}
\end{equation}
%
%
%
\end{proof}


















%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%% Sub - SECTION %%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Proof of Theorem~\ref{thm_Frcht_comp}}
\label{proof_thm_Frcht_comp}

\begin{proof}
    
Since we know that $F_{1}$ is Fr\'echet differentiable at $\boldsymbol{u}$ we have
%
%
%
\begin{equation}\label{eq_proof_thm_Frcht_comp_1}
F_{2}\left( 
       F_{1}\left(
           \boldsymbol{u}
           +
           \boldsymbol{h}
         \right)
       \right)
       = 
       F_{2}
       \left( 
           F_{1}(\boldsymbol{u}) 
           + 
           \bbD_{F_{1}}(\boldsymbol{u})
                 \{ \boldsymbol{h} \} 
                 + 
                 o(\boldsymbol{h}) 
       \right)
       .
\end{equation}
%
%
%
Now, if we take into account the Fr\'echet derivative of $F_{2}\circ F_{1}$ at $\boldsymbol{u}$ we have
%
%
%
\begin{equation}\label{eq_proof_thm_Frcht_comp_2}
F_{2}\left( 
       F\left(
           \boldsymbol{u}
           +
           \boldsymbol{h}
        \right)
       \right)
       = 
       F_{2}\left(
                 F(\boldsymbol{u})
              \right)
           + 
           \bbD_{F_{2}\circ F_{1}}(\boldsymbol{u})
               \{
                  \boldsymbol{h} 
               \} 
               + 
               o(\boldsymbol{h}) 
           ,
\end{equation}
%
%
%
Then, combining~\eqref{eq_proof_thm_Frcht_comp_1} and~\eqref{eq_proof_thm_Frcht_comp_1} and arranging terms we have
%
%
%
\begin{multline}\label{eq_proof_thm_Frcht_comp_3}
\bbD_{F_{2} \circ F_{1}}(\boldsymbol{u})
    \{ 
      \boldsymbol{h} 
     \} 
       =
       \\
              F_{2}
       \left( 
           F_{1}(\boldsymbol{u}) 
            + 
            \bbD_{F_{1}}(\boldsymbol{u})
                \{ 
                  \boldsymbol{h} 
                \} 
            +
            o(\boldsymbol{h}) 
       \right) 
       -
        F_{2}\left(
                 F_{1}(\boldsymbol{u})
               \right)
        -
        o(\boldsymbol{h}) 
        .
\end{multline}
%
%
%
Now, we recall that the Fr\'echet derivative of $F_{2}$ is given according to
%
%
%
\begin{equation}\label{eq_proof_thm_Frcht_comp_4}
F_{2}\left( 
        F_{1}(\boldsymbol{u}) 
        + 
        \boldsymbol{\xi}
      \right)
      =
F_{2}\left( 
        F_{1}(\boldsymbol{u})
      \right)
      +
      \bbD_{F_{2}}\left(
                     F_{1}(\boldsymbol{u})
                  \right) 
                    \{ 
                       \boldsymbol{\xi}
                     \}
      +
      o(\boldsymbol{\xi})
      .
\end{equation}
%
%
%
Then, replacing~\eqref{eq_proof_thm_Frcht_comp_4} in~\eqref{eq_proof_thm_Frcht_comp_3} with $\boldsymbol{\xi} = \bbD_{F_{1}}(\boldsymbol{u})\{ \boldsymbol{h} \} + o(\boldsymbol{h})$ it follows that
%
%
%
\begin{multline}
\bbD_{F_{2} \circ F_{1}}(\boldsymbol{u})
    \{ 
      \boldsymbol{h} 
    \} 
=
\bbD_{F_{2}}\left(
               F_{1}(\boldsymbol{u})
            \right) 
                    \left\lbrace 
                        \bbD_{F_{1}}(\boldsymbol{u})
                             \{ 
                                \boldsymbol{h} 
                              \} 
                        +
                        o(\boldsymbol{h})
                    \right\rbrace
                    \\
                    +
                    o\left( 
                        \bbD_{F_{1}}(\boldsymbol{u})
                           \{ 
                             \boldsymbol{h}
                            \} 
                            +
                            o(\boldsymbol{h})
                     \right)
                     .
\end{multline}
%
%
%
\end{proof}












%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%% Sub - SECTION %%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Proof of Proposition~\ref{prop_derivative_nonlin_and_filter}}
\label{proof_prop_derivative_nonlin_and_filter}



\begin{proof}

Let $F(\boldsymbol{h}) = \boldsymbol{h}\bullet \boldsymbol{x}$, then following the definition of the Fr\'echet derivative we have
%
%
%
\begin{equation}
F\left( 
         \boldsymbol{h}
         +
         \boldsymbol{d}
     \right)    
     -
F\left(
          \boldsymbol{h}
    \right)
    =
    \left( 
          \boldsymbol{h}
          +
          \boldsymbol{d}
    \right)\bullet\boldsymbol{x}
    -
    \boldsymbol{h}
           \bullet
    \boldsymbol{x}
    =
    \boldsymbol{d}
        \bullet
    \boldsymbol{x}
    ,
\end{equation}
%
%
%    
which implies that $\bbD_{F}(\boldsymbol{h})\{ \boldsymbol{d} \} =  \boldsymbol{d} \bullet \boldsymbol{x}$. Now, if we take into account that $\ell (\boldsymbol{h}) = \eta \left( F(\boldsymbol{h})\right)$ and apply the chain rule according to Theorem~\ref{thm_Frcht_comp}, it follows that
%
%
%
\begin{equation}
\bbD_{\ell}(\boldsymbol{h})
         \left\lbrace 
              \boldsymbol{d}  
         \right\rbrace
         =
         \bbD_{\eta}\left( 
                        \boldsymbol{h}
                        \bullet
                        \boldsymbol{x}
                    \right)
                    \left\lbrace 
                         \boldsymbol{d}
                         \bullet
                         \boldsymbol{x}
                    \right\rbrace
                    .
\end{equation}
%
%
%
\end{proof}








% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% %%%%%%%%%%%%%%%%% SUB - SECTION %%%%%%%%%%%%%%%%%
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% \subsection{Proof of Theorem~\ref{thm_one_layer_derivative}}
% \label{proof_thm_one_layer_derivative}

% The proof follows from using the Chain rule in Theorem~\ref{thm_Frcht_comp} and Proposition~\ref{prop_derivative_nonlin_and_filter}.



% \alejandropm{Here write the proof of the simple theorem for one layer}












% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% %%%%%%%%%%%%%%% Sub - SECTION %%%%%%%%%%%%%%%
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% \subsection{Proof of Proposition~\ref{prop_derivative_loss_conv}}
% \label{proof_prop_derivative_loss_conv}



% \begin{proof}

% \begin{multline}
% \ell\left( 
%         \boldsymbol{h}
%         +
%         \boldsymbol{d}
%     \right)
%     -
% \ell(\boldsymbol{h})
% \\
%     =
%     \frac{1}{2}
%          \left\Vert
%            \boldsymbol{r}
%            -
%           \left(
%               \boldsymbol{h}+\boldsymbol{d}
%           \right)\bullet \boldsymbol{x}
%          \right\Vert_{\ccalH(K)}^{2}
%     -
%     \frac{1}{2}
%     \left\Vert
%        \boldsymbol{r}
%        -
%        \boldsymbol{h}\bullet \boldsymbol{x}
%     \right\Vert_{\ccalH(K)}^{2}  
%     .
% \end{multline}
% %
% %
% %
% Now we write the norms in terms of the inner products to obtain
% %
% %
% %
% \begin{multline}
% \ell\left( 
%         \boldsymbol{h}
%         +
%         \boldsymbol{d}
%     \right)
%     -
% \ell(\boldsymbol{h})
% =
% \frac{1}{2}\left\Vert
%                \boldsymbol{r} 
%             \right\Vert_{\ccalH(K)}^{2}
% -
%  \left\langle 
%      \boldsymbol{r}, \boldsymbol{h}\bullet \boldsymbol{x}
%  \right\rangle_{\ccalH(K)}
% -
%  \langle 
%      \boldsymbol{r}, \boldsymbol{d}\bullet \boldsymbol{x}
%  \rangle_{\ccalH(K)}
%  \\
% +
% \frac{1}{2}\left\Vert 
%                \boldsymbol{h}\bullet \boldsymbol{x} 
%             \right\Vert_{\ccalH(K)}^2
% +
% \frac{1}{2}\left\Vert
%                   \boldsymbol{d}\bullet \boldsymbol{x}
%             \right\Vert_{\ccalH(K)}^2
% +
% \left\langle
%    \boldsymbol{d}\bullet \boldsymbol{x}
%    ,
%    \boldsymbol{h}\bullet \boldsymbol{x}
% \right\rangle_{\ccalH(K)}
% \\
%  -
%  \frac{1}{2}\left\Vert 
%                   \boldsymbol{r}
%              \right\Vert_{\ccalH(K)}^2
%  +
%  \left\langle
%          \boldsymbol{r}, \boldsymbol{h}\bullet \boldsymbol{x}
%  \right\rangle_{\ccalH(K)}
%  -
%  \frac{1}{2}\left\Vert 
%                  \boldsymbol{h}\bullet \boldsymbol{x}
%             \right\Vert_{\ccalH(K)}^2
%  ,
% \end{multline}
% %
% %
% %
% Then, canceling out the terms we have
% %
% %
% %
% \begin{multline}
% \ell\left( 
%         \boldsymbol{h}
%         +
%         \boldsymbol{d}
%     \right)
%     -
% \ell(\boldsymbol{h})
% =
%  -
%  \left\langle
%       \boldsymbol{r}
%        ,
%        \boldsymbol{d}\bullet \boldsymbol{x}
%   \right\rangle_{\ccalH(K)}
% +
%   \left\langle
%      \boldsymbol{d}\bullet\boldsymbol{x}
%      ,
%      \boldsymbol{h}\bullet \boldsymbol{x}
%   \right\rangle_{\ccalH(K)}
%   \\
%   +  
%   \left\Vert 
%          \boldsymbol{d}\bullet \boldsymbol{x} 
%   \right\Vert_{\ccalH(K)}^2
% \end{multline}
% %
% %
% %
% Then, we have
% %
% %
% %
% \begin{equation}
% \bbD_{\ell(\boldsymbol{h})}(\boldsymbol{h}) \{ \boldsymbol{d} \} 
%   =
%   \left\langle 
%        \boldsymbol{d}\bullet \boldsymbol{x}
%        ,
%        \boldsymbol{h}\bullet\boldsymbol{x} - \boldsymbol{r}
%   \right\rangle_{\ccalH(K)}
% \end{equation}
% %
% %
% %
% \end{proof}







==> v12/sec_num_exp.tex <==
%!TEX root =../compiler_paper.tex






%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%  S E C T I O N   %%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\section{Numerical Experiments: Learnable Filters in Gphon-SP}
\label{sec:num_exp}


%%-----------------------------------
%%------------ FIGURE ---------------
%%-----------------------------------

\begin{figure*}
%
%--------- FIRST ROW ---------
%
    \centering
       \begin{subfigure}{.32\linewidth}
	   \centering
          \includegraphics[width=1\textwidth]{./figures/fig_num_exp/35_rkhs_regression_result.pdf} 
       \end{subfigure}
    	\begin{subfigure}{.32\linewidth}
		\centering
            \includegraphics[width=1\textwidth]{./figures/fig_num_exp/30_rkhs_regression_result.pdf} 
\end{subfigure}
    	\begin{subfigure}{.32\linewidth}
		\centering
  \includegraphics[width=1\textwidth]{./figures/fig_num_exp/25_rkhs_regression_result.pdf} 
\end{subfigure}
%
%-------- SECOND ROW ---------
%
\centering
\begin{subfigure}{.32\linewidth}
        \centering
        \includegraphics[width=1\textwidth]{./figures/fig_num_exp/20_rkhs_regression_result.pdf} 
        \caption*{$W_{1}(u,v)=u+v$}
\end{subfigure}
\begin{subfigure}{.32\linewidth}
		\centering
            \includegraphics[width=1\textwidth]{./figures/fig_num_exp/15_rkhs_regression_result.pdf} 
            \caption*{$W_{2}(u,v)=\min(x,y)*(1-\max(x,y))$}
\end{subfigure}
\begin{subfigure}{.32\linewidth}
		\centering
            \includegraphics[width=1\textwidth]{./figures/fig_num_exp/10_rkhs_regression_result.pdf} 
            \caption*{$W_{3}(u,v)=1-\max(u,v)$}
\end{subfigure}
    \caption{Reconstruction error of sampled bandlimited signals on graphs derived from a graphon. Each column is associated with experiments performed with a particular graphon, $W_1$ for the left column, $W_2$ for the centered column, and $W_3$ for the column on the right. In the first row, the graphs generated have $250, 500, 750$ and $1000$ nodes. In the second row, the graphs generated have $500, 1000, 1500$ and $2000$ nodes. The graphs are obtained from the graphon using the discretization method (GD1). The bandwidth model considered in this figure is~\textbf{BWM2}. The axis $N$ indicates the number of nodes in the graph. The MSE value depicted is averaged over $50$, which is the number of signals used in each for each reconstruction.}
    \label{fig_error_rec_exp_2}
\end{figure*}

%%--------- End of Figure -----------


==> v12/sec_preliminaries.tex <==
%!TEX root =../compiler_paper.tex





%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%% SECTION %%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\section{Background and Preliminaries}
\leopoldo{We never defined Signal}
In this section, we discuss the preliminaries regarding RKHS and ASP. Before introducing the formal definition of an RKHS, let us state some basic notation. Let $\ccalT$ be a set, and let $\ccalF(\ccalT,\mbF)$ the set of functions from $\ccalT$ to the field $\mbF$. In our discussion we will have either $\mbF=\mbR$ or $\mbF=\mbC$. The set $\ccalF(\ccalT,\mbF)$ is a vector space with the ordinary sum of functions and multiplication of functions by scalars in $\mbF$. When considering any function in $\ccalF(\ccalT,\mbF)$ we use the notation $\boldsymbol{f}(u)$ with $u\in\ccalT$. This will allow us to differentiate when discussing the structure of subspaces of $\ccalF(\ccalT,\mbF)$ and the role of the functions's domain, $\ccalT$. With this notation at hand we formally define RKHS following~\cite{paulsen2016introduction}.



%%-------------------------------------------------
%%------------ D E F I N I T I O N -----------
%%------------------------------------------------

\begin{definition}(\cite{paulsen2016introduction})\label{def_rkhs}
Let $\ccalT$ be a set. Then, $\ccalH\subset \ccalF(\ccalT,\mbF)$ is a reproducing kernel Hilbert space (RKHS) on $\ccalT$ if
%
%
\begin{enumerate}
    %
    %
    \item $\ccalH$ is a vector subspace of $\ccalF(\ccalT,\mbF)$
    %
    %
    \item $\ccalH$ is endowed with an inner product $\langle , \rangle_{\ccalH}$ with respect to which $\ccalH$ is a Hilbert space
    %
    %
    \item For every $u\in\ccalT$, the linear evaluation functional $E_{u}: \ccalH \to \mbF$, defined by $E_{u}(\boldsymbol{f})=\boldsymbol{f}(u)$ is bounded.
    %
    %
\end{enumerate}

\end{definition}

%%------------ End of Definition -------------




If one takes into account the Riez representation theorem~\cite{paulsen2016introduction}, it is possible to show that for any $u\in\ccalT$ there exists a $\boldsymbol{k}_{u}\in\ccalH$ such that $\boldsymbol{f}(u)=\langle \boldsymbol{f}, \boldsymbol{k}_u \rangle_{\ccalH}$ for all $\boldsymbol{f}\in\ccalH$. This also implies that $ E_{u}(f) = \langle \boldsymbol{f}, \boldsymbol{k}_u \rangle_{\ccalH}$. The function $\boldsymbol{k}_u$ allows the definition of a \textit{Kernel} that encapsulates partly the properties of any RKHS. To show this, we introduce first the definition of a Kernel function. 


%%------------------------------------
%%--------- DEFINITION ---------------
%%------------------------------------
\leopoldo{Do we need $K\succcurlyeq 0$ or $K\succ 0$?}
\begin{definition}[\cite{paulsen2016introduction}]
\label{def_kernel}
Let $\ccalT$ be a set and let $K: \ccalT \times \ccalT \to \mbC$ be a function of two variables. Then $K$ is called a kernel function provided that for every $n\in\mbN$ and for every choice of $n$ distinct points, $\{ u_1, \ldots, u_n \}\subset\ccalT$, the matrix $[K(u_i, u_j)]_{i,j}$ is positive semidefinite, which we denote by $[K(u_i, u_j)]_{i,j}\succcurlyeq 0$.
\end{definition}

%%-------- End of Definition ---------


As pointed out in~\cite{paulsen2016introduction}, given an RKHS, $\ccalH$, with evaluation functional $E_{v}(\boldsymbol{f})=\left\langle \boldsymbol{f}, \boldsymbol{k}_{v}(u)\right\rangle_{\ccalH}$, one can obtain a Kernel function, $K(u,v)$, by choosing $K(u,v)=\boldsymbol{k}_{v}(u)$. Additionally, as we will show later $K(u,v)$ allows one to characterize fundamental attributes of the RKHS. We will refer to $K(u,v)=\boldsymbol{k}_{v}(u)$ as the \textit{reproducing kernel} of $\ccalH$. Additionally, from now on, we denote an RKHS by $\ccalH(K)$, emphasizing the reproducing kernel associated with the RKHS. It is worth pointing out that  it is a common practice in the literature,  to start with a kernel function and then find an inner product that allows the definition of an RKHS~\cite{ghojogh2021reproducing,wainwright2019high}.


Now that we have introduced the basics about RKHS we present a classical example of an RKHS that will help us ground these concepts. 


%%------------------------------------------------------------
%%----------------- E X A M P L E  ----------------------
%%------------------------------------------------------------

\begin{example}[Paley Wiener Spaces]\normalfont
\label{exa_rkhs_pw}
%
%
Let $\ccalT = \mbR$ and let $\ccalH(K)$ be given by
%
%
$
 \ccalH(K) 
   =
   \left\lbrace 
       \left.
          \boldsymbol{f}\in C(\mbR)
       \right\vert 
       \text{supp}\left( \widehat{\boldsymbol{f}} \right) \subset [-W, W]
   \right\rbrace 
   ,
$
%
%
where $C(\mbR)$ is the space of continuous functions on $\mbR$ and $\widehat{\boldsymbol{f}}$ is the Fourier transform of $\boldsymbol{f}$. First, we can see that $\ccalH(K)$ is a vector space that can be endowed with the same inner product as in $L_{2}(\mbR)$, i.e.
%
%
%
\begin{equation}
\left\langle 
    \boldsymbol{f},
    \boldsymbol{g}
\right\rangle_{\ccalH(K)}
    =
    \int_{\mbR}\boldsymbol{f}(t)\overline{\boldsymbol{g}(t)}dt
    .
\end{equation}
%
%
%
Taking into account the definition of the inverse Fourier transform we can see that
%
%
%
\begin{equation}
 \boldsymbol{f}(t) 
   =
    \frac{1}{2\pi}
        \int_{-W}^{W}
                \widehat{\boldsymbol{f}}(\omega)e^{j\omega t}
                d\omega
   =
   \frac{1}{2\pi}
    \left\langle
        \widehat{\boldsymbol{f}}
          ,
         e^{-j\omega t}  
    \right\rangle_{\widehat{\ccalH}(W)}
    ,
\end{equation}
%
%
%
where $ \left\langle \cdot , \cdot \right\rangle_{\widehat{\ccalH}(W)}$ is the $L_{2}$ inner product for all the functions supported in $[-W, W]$. Since the Fourier transform defines an isometric transformation we have that
%
%
%
\begin{equation}
 \boldsymbol{f}(t) 
   =
    \frac{1}{2\pi}
    \left\langle
        \widehat{\boldsymbol{f}}
          ,
         e^{-j\omega t} 
    \right\rangle_{\widehat{\ccalH}(W)}
   =
     \left\langle
        \boldsymbol{f}
          ,
        \boldsymbol{k}_{t}
    \right\rangle_{\ccalH(K)}  
    ,
\end{equation}
%
%
%
where 
%
%
$
\boldsymbol{k}_{t}(u)
   =
   \frac{W}{\pi}
      \sinc \left( 
                  \frac{W}{\pi}
                        (u-t)
            \right)
            .
$
%
%
This is, 
%
%
 $
 K(u,t)=   \frac{W}{\pi}
      \sinc \left( 
                  \frac{W}{\pi}
                        (u-t)
            \right)
$
%
%
is the reproducing kernel of $\ccalH(K)$. Using the Cauchy-Schwartz inequality, we have that 
%
%
%
\begin{equation}
    \vert \boldsymbol{f}(t) \vert
        \leq 
            \Vert \boldsymbol{f} \Vert_{\ccalH(K)}
            \Vert \boldsymbol{k}_t \Vert_{\ccalH(K)}
            =
            \Vert \boldsymbol{f} \Vert_{\ccalH(K)}
            \sqrt{\frac{W}{\pi}}
            ,
\end{equation}
%
%
%
which guarantees that $\ccalH(K)$ is an RKHS.
\end{example}

%%----------------- End of Example --------------------



We now proceed to state a collection of results that will help us to characterize any RKHS. This will be of great value in subsequent sections where we study the algebraic properties linked to RKHS. 



%%---------------------------------------------
%%------------ THEOREM -----------------
%%---------------------------------------------

\begin{theorem}(\cite{paulsen2016introduction})\label{thm_density_ky}
Let $\ccalH$ be an RKHS with reproducing kernel $K(u,v)$. Then, the linear span of set of functions $\boldsymbol{k}_{v}(\cdot) = K(\cdot,v)$ for $v\in\ccalT$ is dense in $\ccalH$.
\end{theorem}

%%-------- End of Theorem ----------------



Theorem~\ref{thm_density_ky} highlights the role of the $\boldsymbol{k}_{v} (u)$ functions in an RKHS as an expansion set of functions for any element in $\ccalH$. In a pragmatic scenario,  Theorem~\ref{thm_density_ky} also implies that any element in $\ccalH$ can be approximated with an arbitrary degree of accuracy by a linear combination of functions $\boldsymbol{k}_{v}$. Additionally, since $\boldsymbol{k}_{v}$ is directly obtained from the kernel $K(u,v)$ associated with the RKHS there is a systematic way to generate the functions to approximate any element in $\ccalH$. Now we introduce an example to emphasize this particular point.
 
 
 
%%----------------------------------------------------
%%------------ E X A M P L E  -------------------
%%----------------------------------------------------

\begin{example}\normalfont
\label{ex_pw_space_density_ky}
%
In the context of Example~\ref{exa_rkhs_pw}, we have that the reproducing kernel is $K(u,t)=\frac{W}{\pi}\text{sinc}(W(u-t)/\pi)$. As it is formally shown in~\cite[p.~103] {christensen2016introduction} the set of functions $\boldsymbol{k}_{t}(u)=K(u,t)$ with $t\in\mbZ$ constitutes a basis for the set of bandlimited signals in $[-W,W]$. Then, any bandlimited signal can be written as a linear combination of the $\{ \boldsymbol{k}_{t}(u) \}_{t\in\mbZ}$. The density of $\{ \boldsymbol{k}_{t}(u) \}_{t\in\mbZ}$ emphasizes that to represent some of the elements in $\ccalH(K)$ it might be necessary to use an infinite number of terms in the sum.
%
\end{example}

%%----------- End of Example ------------------




Given an RKHS, $\ccalH(K)$, with kernel $K(u,v)$, one could expect the specific attributes of $K(u,v)$ to influence the functions in $\ccalH(K)$ given the fact that the set of functions $\boldsymbol{k}_{v}(u) = K(u,v)$ is dense in $\ccalH(K)$. This is indeed the case for attributes such as continuity. It can be shown that if $K: \ccalT\times\ccalT\to\mbF$ is continuous -- considering the product topology -- then every function in $\ccalH(K)$ is continuous -- see Theorem 2.17 in~\cite{paulsen2016introduction} --, and where the notion of continuity in $\ccalH(K)$ is tied to the topology of $\ccalT$. Such association between the properties of $K$ and those of $\ccalH(K)$ is also strenghtened by the fact that any kernel $K:\ccalT\times\ccalT\to\mbF$ induces a unique RKHS -- Theorem 2.14 in~\cite{paulsen2016introduction} --.







%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%  SUB - SECTION  %%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{RKHS and Integral Operators}
\label{sub_sec_rkhs_int_oper}

In this section, we discuss an important family of RKHS where the underlying kernel has properties characterized by an integral operator. In particular, we are interested in integral operators, $T_{S}$, given by
%
%
%
\begin{equation}\label{eq_sub_sec_rkhs_int_oper_1}
T_{S}\left\lbrace 
        \boldsymbol{f}
 \right\rbrace
        =
        \int_{\ccalT}
             S(u,v)\boldsymbol{f}(v)d\mu(v),
\end{equation}
%
%
%
where $S: \ccalT\times\ccalV \to \mbC$ is square integrable as a function of $v$, for any $u\in\ccalT$. The symbol $\mu$ is a measure on $\ccalV$. Then, for a given integral operator, $T_{S}$, we will refer to $S$ as the \textit{symbol} of $T_{S}$. When considering two symbols, $S_{1}(u,v)$ and $S_{2}(u,v)$, one can use the \textit{box product} to produce another symbol with desirable properties~\cite{paulsen2016introduction}. If we denote by $\square$ the box product between $S_{1}(u,v)$ and $S_{2}(u,v)$, we have
%
%
%
\begin{equation}\label{eq_box_product}
 \left(
     S_{1}\square S_{2}
 \right)(u,v)
       =
       \int_{\ccalY}
             S_{1}(u,z)
             S_{2}(z,v)
                 d\mu (z)
                 .
\end{equation}
%
%
%
This operation is beneficial to build kernels -- in the sense of Definition~\ref{def_kernel} --. In fact,  if $S^{\ast}(u,v)=\overline{S(v,u)}$, then $S\square S^{\ast}$ is a kernel function~\cite[Theorem~11.2]{paulsen2016introduction}. Additionally, from~\cite{paulsen2016introduction} -- Proposition 2.13 -- we know that given a kernel $K(u,v)$, we can associate to it a unique RKHS, $\ccalH(K)$. 



Among the kernels whose properties can be related to integral operators are \textit{Mercer kernels}, which are \textit{continuous} kernel functions. Given its importance we state formally their definition as follows.


%%---------------------------------------
%%------------ DEFINITION ---------------
%%---------------------------------------

\begin{definition}[\cite{paulsen2016introduction}]
\label{def_mercer_kernel}
%
Let $\ccalT$ be a compact subset of $\mbR^{N}$. A function $K: \ccalT\times\ccalT \to \mbC$ is called a Mercer kernel if it is a continuous, positive semidefinite function, i.e. a continuous kernel function. 
%
\end{definition}

%%--------- End of Definition -----------




For Mercer kernels, we can write $K$ as a decomposition in terms of the spectral decomposition of an associated integral operator. This point is emphasized in the following result. 



%%--------------------------------------
%%------------- THEOREM ----------------
%%--------------------------------------

\begin{theorem}[\cite{paulsen2016introduction}]
\label{thm_mercer}
%
Let $K$ be a Mercer kernel on $\ccalT$, let $\mu$ be a finite Borel measure with support $\ccalT$, and let $T_{K}: L_{2}(\ccalT,\mu)\to L_{2}(\ccalT,\mu)$ be the associated integral operator -- as in~\eqref{eq_sub_sec_rkhs_int_oper_1} --. Then there is a countable collection of orthonormal continuous functions $\{ \boldsymbol{\varphi}_i \}_{i=1}^{\infty}$ on $\ccalT$ that are eigenvectors for $T_{K}$ with corresponding eigenvalues $\{ \sigma_i \}_{i=1}^{\infty}$ such that for every $\boldsymbol{g}\in L_{2}(\ccalT,\mu)$ we have
%
%
%
\begin{equation}
T_{K}\{ \boldsymbol{g} \}
      =
      \sum_{i=1}^{\infty}
             \sigma_{i}
                  \left\langle
                        \boldsymbol{g}
                        ,
                        \boldsymbol{\varphi}_i
                  \right\rangle_{L_{2}}
                  \boldsymbol{\varphi}_{i}
                  .
\end{equation}
%
%
%
Furthermore,
%
%
%
\begin{equation}\label{eq_mercer_K_decomp}
K(u,v)
     =
      \sum_{i=1}^{\infty}
            \sigma_{i}
            \boldsymbol{\varphi}_{i}(u)
            \boldsymbol{\varphi}_{i}(v)
            .
\end{equation}
%
%
%
\end{theorem}

%%---------- End of Theorem ------------




Theorem~\ref{thm_mercer} provides us with the tools to characterize an RKHS in terms of an operator that can be leveraged to define convolutional signal models -- we will get to this point in Section~\ref{sec_conv_filt_rkhs}. Additionally, notice that the RKHS associated with the kernel in~\eqref{eq_mercer_K_decomp} is 
%
%
%
\begin{equation}\label{eq_HK_in_L2_as_rkhs}
\ccalH(K)
=
\left\lbrace 
       \boldsymbol{f}\in L_{2}(\ccalT,\mu)
    \left\vert
        \sum_{i=1}^{\infty}
             \frac{
                   \langle
                      \boldsymbol{f}
                      ,
                      \boldsymbol{\varphi}_i
                   \rangle_{L_{2}}^{2}
                  }
                  {\sigma_i}
                  <
                  \infty
    \right.              
\right\rbrace
,
\end{equation}
%   
%
%
with inner product given by
%
%
%
\begin{equation}\label{eq_H_innerprod_vs_L2}
\left\langle
    \boldsymbol{f}
    ,
    \boldsymbol{g}
\right\rangle_{\ccalH(K)}
    =
    \sum_{i=1}^{\infty}
        \frac{
              \left\langle
                   \boldsymbol{f}
                   ,
                   \boldsymbol{\varphi}_i
              \right\rangle_{L_2}
              \left\langle
                   \boldsymbol{g}
                   ,
                   \boldsymbol{\varphi}_i
              \right\rangle_{L_2}
             }
        {\sigma_i}
        .
\end{equation}
%
%
%
We refer the reader to Appendix~\ref{sub_sec_Ts_Tk_relationship} for details on how these derivations are obtained. 




%%------------------------------------
%%------------ EXAMPLE ---------------
%%------------------------------------

\begin{example}\normalfont
%
One of the essential ingredients of a Mercer kernel -- see Definition~\ref{def_mercer_kernel} -- is the compactness of the domain of the functions, $\ccalT$. One could, in principle, start with a kernel, $K$, defined on an arbitrary $\ccalT$, and then restrict $K$ to a compact subset $\ccalC\subset\ccalT$ to build a Mercer kernel. As pointed out in~\cite[p.~396-399]{wainwright2019high} this is the case. For instance, using the kernel $K(u,t)=\frac{W}{\pi}\text{sinc}(W(u-t)/\pi)$ from Example~\ref{ex_pw_space_density_ky} or the Gaussian kernel $K(u,t)=\exp{\left(-(u-t)^{2}/(2\sigma^2) \right)}$, we obtain Mercer kernels using the restriction $u,t\in [-1,1]$. Notice that while imposing the restriction of the domain on the kernel guarantees that we have a Mercer kernel, it may not be trivial to obtain the decomposition in~\eqref{eq_mercer_K_decomp} for those kernels that are originally defined in non compact domains. This can be observed in~\cite{widomgaussnkernel} and~\cite{Bonami2018NonAsymptoticBO} for the Gaussian and the Sinc kernel in $[-1,1]$, where only estimates of the asymptotic behavior can be determined for the spectral decompositions as in~\eqref{eq_mercer_K_decomp}.
%
\end{example}

%%--------- End of Example -----------



We know that when considering symbols and integral operators, we can build a kernel using the box product. If we also restrict to continuous symbols on compact domains, we obtain a Mercer kernel. While not obvious, one can expect to start with a Mercer kernel and then obtain a symbol that can be used to build a convolutional model. This observation is formalized in the following theorem from~\cite{paulsen2016introduction}.



%%---------------------------------------------------------------
%%------------------ T H E O R E M -----------------------
%%---------------------------------------------------------------

\begin{theorem}[Theorem 11.18 in~\cite{paulsen2016introduction}]
\label{thm_S_from_K_rkhs}
%
Let $K$ be a Mercer kernel on $\ccalT$, let $\mu$ be a finite Borel measure with support $\ccalT$ and let $\{ \boldsymbol{\varphi}_i \}$ be the orthonormal family of eigenvectors corresponding to non zero eigenvalues $\{ \sigma_i \}$ of $T_{K}$ given by Theorem~\ref{thm_mercer}. Then:
%
%
\begin{enumerate}
  %
  \item $S(u,v)=\sum_{i}\sqrt{\sigma_i}\boldsymbol{\varphi}_{i}(u)\boldsymbol{\varphi}_{i}(v)$ is the symbol of a bounded integral operator, $T_{S}$, on $L_{2}(\ccalT,\mu)$;
  %  
  \item $T_{S}$ is a positive operator with $T_{S}^{2} = T_{K}$;
  %
  \item $\{ \sqrt{\lambda_i}\boldsymbol{\varphi}_{i} \}$ is an orthonormal basis for $\ccalH(K)$;
  %
  \item $\ccalH(K)$ consists precisely of the functions $\sum_{i}\alpha_{i}\boldsymbol{\varphi}_{i}(u)$ such that 
  %
  $
  \sum_{i}\left(\vert \alpha_{i}\vert^{2}/\lambda_{i}\right)<\infty.
  $
  %
\end{enumerate}
%
%
\end{theorem}

%%---------- End of Theorem -------------


Finally, we remark that, as we will show in subsequent sections, graphon signal processing is one of those scenarios where the symbol associated with the kernel in an RKHS, defines the attributes of a signal model, in particular the attributes of a graph-like domain whose number of nodes and edges is infinite. 



==> v12/sec_rkhs_nn.tex <==
%!TEX root =../compiler_paper.tex





%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%% SECTION %%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\section{Algebraic RKHS Neural Networks}
\label{sec_alg_rkhs_nn}


In this section, we describe convolutional neural networks based on RKHS. To formally leverage the structure induced by an RKHS, we exploit algebraic neural networks (AlgNNs), introduced in~\cite{parada_algnn, parada_algnnconf, algnn_nc_j} to describe general convolutional neural networks.


An AlgNN is a stacked layered structure. Information is processed in each layer employing a convolutional operator, a pointwise nonlinearity, and a pooling operator -- see Fig.~\ref{fig_rkhs_nn_one_layer} --. In the following subsections, we describe the details of each of these operators.


%%-------------------------------------------
%%-----------  F I G U R E  -------------
%%-------------------------------------------

\begin {figure}
\centering
\input{figures/algnn_one_layer.tex}
%
\caption{Structure of one layer of an RKHS neural network. The signal $\boldsymbol{y}_{\ell}$ is the result of filtering $\boldsymbol{x}_{\ell-1}\in\ccalH(K)$ with an element from $\ccalA_{\ccalH(K)}$ according to the ASM in~\eqref{eq_rkhs_asm_standard}. A pointwise nonlinearity operator $\eta_{\ell}: \ccalH(K)\to \ccalH(K)$ is applied to $\boldsymbol{y}_{\ell}$ to obtain $\boldsymbol{z}_{\ell}$ and a pooling operator $P_{\ell}$ performs dimensionality reduction on $\boldsymbol{z}_{\ell}$ to obtain a signal $\boldsymbol{x}_{\ell}$ that can be fed into another layer.} 
%
\label{fig_rkhs_nn_one_layer}
\end{figure}

%%------- E N D  of Figure  ---------






%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%% SUB - SECTION %%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{The convolutional operator}

The convolutional operator is defined according to a specific ASM. For our discussion the ASM model considered is $(\ccalA_{\ccalH}, \ccalH(K), \rho)$, where $\ccalH(K)$ is an RKHS, $\ccalA_{\ccalH}$ is the algebra induced by $\ccalH(K)$ -- see Theorem~\ref{thm_general_A_rkhs} -- and $\rho$ translates the action of the filters in $\ccalA_{\ccalH}$ into product operators that rely on the $\bullet$ product in $\ccalA_{\ccalH}$. Then, if $\boldsymbol{x}_{\ell-1}\in\ccalH(K)$ is the input signal to the layer $\ell$ of the AlgNN, the result of applying the convolutional operator 
%
%
$
\sum_{k}h_{\ell,k}\boldsymbol{k}_{g_1}^k
$
%
%
is given by
%
%
%
\begin{equation}
\displaystyle{\boldsymbol{y}_{\ell}  = \sum_{r}h_{\ell,r}\boldsymbol{k}_{g_r}^{\bullet r}} \bullet\boldsymbol{x}_{\ell-1}   
,
\end{equation}
%
%
%
where $\boldsymbol{k}_{g_r}^{\bullet r}$ is the $r$-times product ``$\bullet$" of $\boldsymbol{k}_{g_r}$. Notice that the action of $\bullet$ on $\boldsymbol{x}_{\ell}$ is given by~\eqref{eq_A_rkhs_gen_prod} since $\boldsymbol{x}_{\ell-1}\in\ccalH(K)$.






%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%% SUB - SECTION %%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{The pointwise nonlinearity}
\label{sub_sec_nonlinearity}

The point-wise nonlinearity is defined as an operator $\eta_{\ell}: \ccalH(K) \to \ccalH(K)$ whose action is \textit{point-wise} in terms of a specific basis~\cite{parada_algnn}. A fundamental assumption on $\eta_{\ell}$ is that the images of $\eta_{\ell}$ are indeed in $\ccalH(K)$. This has a strong implication on the implementation aspects of $\eta_\ell$. To see this, consider for instance that one wishes to use the ReLu as a pointwise nonlinearity. Then, one has to guarantee that the images of the operator $\max\{ 0, \boldsymbol{f}(u) \}$ are in $\ccalH$ which is an RKHS. Naturally, this is not always the case and an additional projection operation could be necessary to map information inside $\ccalH(K)$. To guarantee that the images of $\eta_\ell$ are in $\ccalH (K)$ we leverage Theorem~\ref{thm_density_ky}. Then, since the functions, $\boldsymbol{k}_{v}(u)$, constitute a dense set in $\ccalH(K)$, 
any element in $\ccalH(K)$ can be written as $\boldsymbol{y}_{\ell} = \sum_{v\in\ccalV}\alpha_{v}\boldsymbol{k}_{v}$ with $\ccalV\subset\ccalT$. Therefore, the action of $\eta_{\ell}$ can be written as
%
%
%
\begin{equation}\label{eq_nonlinearity_a} 
\boldsymbol{z}_{\ell}(t)
     =
     \eta_{\ell}
           \left( 
                \boldsymbol{y}_{\ell}(t)
           \right)
    =
    \sum_{v\in\ccalV}
        \widehat{\eta}_{\ell,v}\left( \boldsymbol{y}_{\ell}(t) \right)   
        \boldsymbol{k}_{v}(t)  
        ,
\end{equation}
%
%
%
where $\widehat{\eta}_{\ell,v}: \ccalH(K) \to \mbF$. For the selection of $\widehat{\eta}_{\ell,v}$ we choose a map that ensures the continuity concerning the localization of the $\boldsymbol{k}_{v}(t)$. To this end, we make the following selection
%
%
%
\begin{equation}\label{eq_nonlinearity_b}
\widehat{\eta}_{\ell,v}
        \left( 
                \boldsymbol{y}_{\ell}(t)
        \right)
=
\frac{
       \sigma\left( \boldsymbol{y}_{\ell}(v) \right)
      }
      {
      \sum_{r\in\ccalV}\boldsymbol{k}_{v}(r)
      }
      ,
\end{equation}
%
%
%
where $\sigma (x) = \max\{ 0, x \}$ is the traditional ReLu function. In Appendix~\ref{sub_sec_cont_pointwisenonl}, we show formally that $\eta_{\ell}$ is continuous besides the choice of $\sigma$.



% we can define the action of a pointwise nonlinearity on the coefficients of a representation written in terms of the  $\boldsymbol{k}_{v}(u)$. This will also guarantee that the images of $\eta_{\ell}$ are in $\ccalH(K)$.

% the representation of $K(u,v)$ in terms of a basis -- see Theorem~\ref{thm_K_from_basis_general} -- and define the action of $\eta_{\ell}$ on the coefficients of the representation in terms that basis. More specifically, since the span of $\boldsymbol{k}_y$ is dense in $\ccalH$ -- see Theorem~\ref{thm_density_ky} -- any element in $\ccalH$ can be approximately written as $\boldsymbol{y}_{\ell} = \sum_{x}\alpha_{x}\boldsymbol{k}_{x}$. Then, if $K(x,y)=\sum_{s\in\ccalS}\overline{e_{s}(x)}e_{s}(y)$, it follows that
% %
% %
% %
% \begin{equation}
%  \boldsymbol{y}_{\ell}(t)
%      = 
%      \sum_{x}\alpha_{x}
%              \boldsymbol{k}_{x}(t) 
%      =
%      \sum_{s\in\ccalS}
%           \left(
%                 \sum_{x}
%                      \alpha_{x}\boldsymbol{e}_{s}(x)
%           \right)\boldsymbol{e}_{s}
%           .
% \end{equation}
% %
% %
% %
% Then, any point-wise non-linearity $\eta_{\ell}:\ccalH \to \ccalH$ can be defined as an operator that acts on the coefficients of the expansion in terms of the expansion obtained from the $\boldsymbol{e}_{s}$. This is,
% \blue{
% %
% %
% %
% \begin{equation}
% \boldsymbol{z}_{\ell}(t)
%      =
%      \eta_{\ell}
%            \left( 
%                 \boldsymbol{y}_{\ell}(t)
%            \right)
% \end{equation}
% %
% %
% %
% }
% %
% %
% %
% \begin{equation}\label{eq_nonlinearity_a}
% \boldsymbol{z}_{\ell}(t)
%      =
%      \eta_{\ell}
%            \left( 
%                 \boldsymbol{y}_{\ell}
%            \right)
%       =
%      \sum_{s\in\ccalS}
%           \widehat{\eta}_{\ell}\left(
%                 \sum_{x}
%                      \alpha_{x}\boldsymbol{e}_{s}(x)
%           \right)\boldsymbol{e}_{s} 
%         ,
% \end{equation}
% %
% %
% %
% where $\widehat{\eta}_{\ell}: \mbR \to \mbR$ is an ordinary real-valued function of one independent variable. Notice that the value
% %
% %
% $
% \eta_{\ell}\left(
%                 \sum_{x}
%                      \alpha_{x}\boldsymbol{e}_{s}(x)
%            \right)\in\mbR
% $
% %
% %
% is indexed by $s$.

% Notice that the description of $\eta_{\ell}$ allows for a rich selection of pointwise nonlinearities whose effectiveness can be studied in future research works. For our numerical implementations, we will use the sub-family of nonlinearities characterized by
% %
% %
% %
% \begin{equation}\label{eq_nonlinearity_b}
% \widehat{\eta}_{\ell}\left(
%                 \sum_{x}
%                      \alpha_{x}\boldsymbol{e}_{s}(x)
%            \right)
%            =
%            \sum_{x}
%                 \widehat{\eta}_{\ell}
%                      \left( 
%                           \alpha_x
%                      \right)
%                      \boldsymbol{e}_{s}(x)
%                      .
% \end{equation}
% %
% %
% %





%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%% SUB - SECTION %%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{The pooling operator}
\label{sub_sec_pooling}

Pooling is meant to reduce the complexity of the signals while preserving its essential structure~\cite{deeplearning_book,boureau_pooling_1}. As shown in~\cite{algnn_nc_j,parada_algnn}, the description of a pooling operator in an AlgNN can be achieved by leveraging a basis representation on the spaces involved. Then, a typical pooling operator, $P_{\ell}$, reduces the complexity of the signal by reducing the number of elements in the basis considered for the representation of the signal. Then, taking into account the representation of any element of $\ccalH(K)$ in terms of the $\boldsymbol{k}_{v}(u)$, we have
%
%
%
\begin{equation}
P_{\ell}\left( 
           \sum_{s\in\ccalS_{\ell}}
                  \alpha_{s}
                  \boldsymbol{k}_{s}
        \right)
        =
        \sum_{s\in\ccalS_{\ell+1}}
                  \alpha_{s}
                  \boldsymbol{k}_{s}
                  ,
\end{equation}
%
%
%
where $\ccalS_{\ell+1}\subset\ccalS_{\ell}$ with $\vert \ccalS_{\ell+1}\vert < \vert \ccalS_{\ell}\vert$.











%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%% SUB - SECTION %%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Training and Learnable Parameters}

%%----------------------------------------------
%%------------  F I G U R E  ---------------
%%----------------------------------------------

\begin{figure*}
%
%
\centering
	\centering
 \input{./figures/fig_1_source_tikz.tex} 
%
%
\caption{Depiction of the RKHS architecture considered for our experiments considering. In the first layer two layers ($N_{1}=2$) are followed by a pointwise nonlinearity operator. The outputs from the first layer are fed into a second layer with two filters per input ($N_{2}$). Then, the output of each filter group are summed up and processed with a pointwise nonlinearity operator. The outputs from the second layer are added up to obtain the output, $\boldsymbol{y}$.}
\label{fig:simulation_network}
\end{figure*}

%%--------- End of Figure -----------




The learnable parameters in the RKHS-based network are the filters used in each layer of the network -- which are elements of $\ccalA_{\ccalH}$ in Theorem~\ref{thm_general_A_rkhs}. Since such filters can be written in terms of the functions $\boldsymbol{k}_{v}$ in the RKHS, we end up in a scenario where we learn the coefficients in that representation as well as the subindices, $v$.


We use a gradient descent approach to find the optimal filters that minimize the square quadratic error in the training of the RKHS network. While this computation is analogous to that one performed for finite-dimensional spaces, there are differences. In particular, the gradient descent in the RKHS network involves functional optimization and therefore the use of Fr\'echet derivatives. In what follows, we derive explicit expressions to illustrate how this process takes place. To this end, we consider the RKHS network in Figure~\ref{fig:simulation_network}. Please notice that this is just one particular example of an RKHS network that we will consider later for our numerical experiments, but the theory and discussions presented above are valid for different network topologies.  


In Fig.~\ref{fig:simulation_network}, we have an RKHS network where the learnable parameters are filters in $\ccalA_{\ccalH(K)}$. We have two layers. In the first layer, we have a total of $N_1$ filters, $\left\lbrace \boldsymbol{h}_{j}^{(1,0)} \right\rbrace_{j=1}^{N_1}$, each followed by a point-wise non-linearity, $\eta(\cdot)$. Then, the features obtained are fed into a second layer, where we have $N_2$ filters, $\left\lbrace \boldsymbol{h}_{j}^{(2,i)} \right\rbrace_{i=1}^{N_2}$, per each feature -- each $j$ -- coming from layer one. We add up the output of those $N_2$ filters -- per each feature coming from the first layer, i.e. each $j$ -- and then apply a pointwise nonlinearity, $\eta(\cdot)$. Then, we add all the resultant signals again to obtain the final output of the network, which belongs to $\ccalH(K)$. For an input, $\boldsymbol{x}$, the network produces an output, $\boldsymbol{y}$, given by
%
%
%
\begin{equation}\label{eq_input_output_rel_network}
\boldsymbol{y}
=
\sum_{i=1}^{N_2}
  \eta\left(
         \sum_{j=1}^{N_1}
              \boldsymbol{h}_{j}^{(2,i)}
                   \bullet
               \eta\left(
                       \boldsymbol{h}_{j}^{(1,0)}
                            \bullet
                       \boldsymbol{x}     
                   \right)
   \right) 
   .
\end{equation}
%
%
%

Then, our goal when training the network is to find the filters in~\eqref{eq_input_output_rel_network} that minimize the quadratic error, measured when comparing the output of the network to the given input and reference signals. To show this explicitly, let us rewrite~\eqref{eq_input_output_rel_network} as 
%
%
%
\begin{equation}\label{eq_input_output_rel_network_2}
 \boldsymbol{y}
     =
      F\left(
           \boldsymbol{h}_T
       \right)
       ,
\end{equation}
%
%
%
with 
%
%
%
\begin{equation}
\boldsymbol{h}_{T}
    =
\left( 
    \left(
        \boldsymbol{h}_{j}^{1,0}
    \right)_{j=1}^{j=N_1}
    ,
    \left(
        \boldsymbol{h}_{j}^{2,i}
    \right)_{j=1,i=1}^{j=N_1,i=N_2}  
\right)
.
\end{equation}
%
%
%

Then, given an input $\boldsymbol{x}$ to the RKHS network and a reference signal $\boldsymbol{r}\in \ccalH(K)$ we aim to minimize 
%
%
%
\begin{equation}\label{eq_ell_Fh}
\ell(\boldsymbol{h}_{T})
        =
         \frac{1}{2}
            \left\Vert
                  \boldsymbol{r}
                  -
                    F\left(
                         \boldsymbol{h}_{T}
                      \right)
            \right\Vert_{\calH(K)}^2
            .
\end{equation}
%
%
%

In order to write explicit expressions for gradient descent we require the calculation of the Fr\'echet derivative of 
%
%
$      
F\left(
      \boldsymbol{h}_T
  \right)
  .
$ 
%
%
We can achieve this by taking into account that
%
%
%
\begin{equation}
 F
 \left(
      \boldsymbol{h}_T
  \right)
     =
F^{(1)}
   \left(
       \boldsymbol{h}_{j}^{(1,0)}
   \right) 
   =
F^{(2)}   
   \left(
       \boldsymbol{h}_{j}^{(2,i)}
   \right) 
   ,
\end{equation}
%
%
%
where the expression of $F^{(1)}$ coincides with the expression of $F$ with the terms $\boldsymbol{h}_{j}^{(2,i)}$ constant. Analogously, the expression of $F^{(2)}$ coincides with the expression of $F$ with the terms $\boldsymbol{h}_{j}^{(1,0)}$ constant. Then, by means of the Fr\'echet derivative properties -- see~\cite{berger1977nonlinearity} pages 69-71 -- we have 
%
%
%
\begin{multline}
\bbD_{F}\left(
           \boldsymbol{h}_{T}
        \right)
     \left\lbrace 
          \boldsymbol{d}_{T}
     \right\rbrace
     =
     \sum_{j=1}^{N_1}\bbD_{F^{(1)}}
             \left( 
                  \boldsymbol{h}_{j}^{(1,0)}
             \right)
                  \left\lbrace 
                       \boldsymbol{d}_{j}^{1,0}
                  \right\rbrace
      +            
      \\            
       \sum_{j=1}^{N_1}
       \sum_{i=1}^{N_2}\bbD_{F^{(2)}}
             \left( 
                  \boldsymbol{h}_{j}^{(2,i)}
             \right)
                  \left\lbrace 
                       \boldsymbol{d}_{j}^{(2,i)}
                  \right\rbrace
                  ,
\end{multline}
%
%
%
where

%
%
%
\begin{equation}
\boldsymbol{d}_{T}
    =
\left( 
    \left(
        \boldsymbol{d}_{j}^{1,0}
    \right)_{j=1}^{j=N_1}
    ,
    \left(
        \boldsymbol{d}_{j}^{2,i}
    \right)_{j=1,i=1}^{j=N_1,i=N_2}  
\right)
.
\end{equation}
%
%
%


In the following Theorem, we derive explicit expressions for the Fr\'echet derivatives of $F^{(1)}$ and $F^{(2)}$. 





%%--------------------------------------
%%------------- THEOREM ----------------
%%--------------------------------------

\begin{theorem}\label{thm_F1_F2_derivatives}
%
Let $\ccalH(K)$ be an RKHS with reproducing kernel $K(u,v)$ and let $F^{(1)}:\ccalH(K) \to \ccalH(K)$ and $F^{(2)}:\ccalH(K) \to \ccalH(K)$ be given by
%
%
%
\begin{multline}
 F^{(1)}\left(
      \boldsymbol{h}_{j}^{(1,0)}
  \right)  
  =
\sum_{i=1}^{N_2}
  \eta\left(
         \sum_{j=1}^{N_1}
              \boldsymbol{h}_{j}^{(2,i)}
                   \bullet
               \eta\left(
                       \boldsymbol{h}_{j}^{(1,0)}
                            \bullet
                       \boldsymbol{x}     
                   \right)
   \right)  
   ,
\end{multline}
%
%
%
and
%
%
%
\begin{multline}
 F^{(2)}\left(
            \boldsymbol{h}_{j}^{(2,i)}
        \right)  
  =
\sum_{i=1}^{N_2}
  \eta\left(
         \sum_{j=1}^{N_1}
              \boldsymbol{h}_{j}^{(2,i)}
                   \bullet
               \eta\left(
                       \boldsymbol{h}_{j}^{(1,j)}
                            \bullet
                       \boldsymbol{x}     
                   \right)
   \right)  
   .
\end{multline}
%
%
%






Then, it follows that
%
%
%
\begin{multline}
\bbD_{F^{(1)}}\left(
         \boldsymbol{h}_{j}^{(1,0)}
      \right)
     \left\lbrace
        \boldsymbol{d}_{j}^{(1,0)} 
     \right\rbrace
     =
     \\
      \sum_{i=1}^{N_2}
            \bbD_{\eta}
                 \left( 
                     \boldsymbol{h}_{j}^{(2,i)}
                        \bullet
                      \boldsymbol{h}
                      +
                      \sum_{k\neq j}
                           \boldsymbol{h}_{k}^{(2,i)}
                           \bullet
                           \eta\left( 
                                  \boldsymbol{h}_{k}^{(1,0)}
                                    \bullet
                                  \boldsymbol{x}
                               \right)
                 \right)
                 \\
                    \left\lbrace 
                        \boldsymbol{h}_{j}^{(2,i)} 
                          \bullet
                                 \bbD_{\eta}\left( 
                       \boldsymbol{h}_{j}^{(1,0)}
                            \bullet
                        \boldsymbol{x}
                    \right)
                          \left\lbrace 
                               \boldsymbol{d}_{j}^{(1,0)} 
                               \bullet
                               \boldsymbol{x}
                          \right\rbrace
                    \right\rbrace
                    ,
\end{multline}
%
%
%
%
%
%
\begin{multline}
\bbD_{F^{(2)}}
          \left(
               \boldsymbol{h}_{j}^{(2,i)}
          \right)
    \left\lbrace 
        \boldsymbol{d}_{j}^{(2,i)}
    \right\rbrace
    =
    \\
    \bbD_{\eta}\left(
                    \boldsymbol{h}_{j}^{(2,i)}
                       \bullet
                    \eta\left(
                           \boldsymbol{h}_{j}^{(1,0)}
                              \bullet
                           \boldsymbol{x}   
                        \right)
                    +
                    \sum_{k\neq j}
                        \boldsymbol{h}_{k}^{(2,i)}
                             \bullet
                        \eta\left( 
                                \boldsymbol{h}_{j}^{(1,0)}
                                   \bullet
                                \boldsymbol{x}   
                            \right)
                \right)
                \\
      \left\lbrace 
          \boldsymbol{d}_{j}^{(2,i)}
              \bullet
          \eta\left( 
                   \boldsymbol{h}_{j}^{(1,0)}
                      \bullet
                   \boldsymbol{x}   
              \right)
      \right\rbrace
      .
\end{multline}
%
%
%
\end{theorem}

\begin{proof}
    See Appendix~\ref{proof_thm_F1_F2_derivatives}.
\end{proof}


%%---------- End of THEOREM ------------



In what follows we derive concrete expressions for the derivatives of the pointwise non-linearities, $\bbD_{\eta}(\boldsymbol{h})\{ \boldsymbol{d} \}$, taking into account the considerations discussed in Section~\ref{sub_sec_nonlinearity}.



%%---------------------------------------
%%------------- THEOREM -----------------
%%---------------------------------------

\begin{theorem}\label{thm_frechet_nonlinearity}
%
Let $\ccalH(K)$ be an RKHS with reproducing kernel $K(u,v)$ and let $\eta: \ccalH(K)\to \ccalH(K)$ be a point-wise non-linearity as specified in~\eqref{eq_nonlinearity_a} and~\eqref{eq_nonlinearity_b}. Then, the Fr\'echet derivative of $\eta$ evaluated at 
%
%
%
\begin{equation}
\displaystyle\boldsymbol{h}=
             \sum_{u\in\ccalU_1}\bbh(u)\boldsymbol{k}_{u}    
\end{equation}
%
%
%
and acting on
%
%
%
\begin{equation}
 \boldsymbol{d}=
          \sum_{u\in\ccalU_2}\bbd(u)\boldsymbol{k}_{u}   
\end{equation}
%
%
%
is given by
%
%
%
\begin{equation}\label{eq_thm_frechet_nonlinearity_1}
 \bbD_{\eta}(\boldsymbol{h})
          \left\lbrace 
                 \boldsymbol{d}
          \right\rbrace 
          =
          \sum_{u\in\ccalU}
                     \frac{
    \sigma^{'}\left(
                  \boldsymbol{h}(u)
              \right)
              \boldsymbol{d}(u)
    }
    {
     \sum_{r,u\in\ccalU}\boldsymbol{k}_{u}(r)
    }
                 \boldsymbol{k}_{u}     
          ,
\end{equation}
%
%
%
where $\ccalU = \ccalU_1 \bigcup \ccalU_2$ and $\sigma^{'}$ is the ordinary derivative of $\sigma$.
\end{theorem}

\begin{proof}
    See Appendix~\ref{proof_thm_frechet_nonlinearity}
\end{proof}

%%--------- End of Theorem --------------



Notice that the expression in~\eqref{eq_thm_frechet_nonlinearity_1} does not require $\boldsymbol{h}$ and $\boldsymbol{d}$ being represented with $\ccalU_1 = \ccalU_2$. 

We now state the expression that defines the derivative of the cost function, $\ell(\boldsymbol{h})$, in terms of $F(\boldsymbol{h})$ in~\eqref{eq_ell_Fh}. This will be of essential importance to state the steepest descend formulation of the problem.


	

%%------------------------------------------
%%------------- PROPOSITION ----------------
%%------------------------------------------

\begin{prop}\label{prop_derivative_loss_Fh}
%
Let $\ccalH(K)$ be an RKHS with reproducing kernel $K$. Given a reference signal $\boldsymbol{r}\in \mathcal H(K)$, a filter $\boldsymbol{h}\in \ccalA_{\ccalH(K)}$ -- see Theorem~\ref{thm_general_A_rkhs} --  and define $\ell(\boldsymbol{h}):\mathcal H(K)\to \mathbb R$ as 
%
%
$
\ell(
    \boldsymbol{h}
    )
    =\frac{1}{2}
         \left\Vert 
               \boldsymbol{r}
               -
               F\left(
                    \boldsymbol{h}
                \right)    
         \right\Vert_{\calH(K)}^2
,
$
%
%
where $F:\ccalH(K)\to\ccalH(K)$ is Fr\'echet differentiable. Then,
%
%
%
\begin{equation}
\bbD_{\ell}(\boldsymbol{h})
     \left\lbrace 
           \boldsymbol{d}
     \right\rbrace
     =
     -
     \left\langle 
           \bbD_{F}(\boldsymbol{h})\left\lbrace 
                                        \boldsymbol{d} 
                                   \right\rbrace
           ,  
           \boldsymbol{r}
           -
           F(\boldsymbol{h})
    \right\rangle_{\ccalH(K)}
    .
\end{equation}
%
%
%
\end{prop}

\begin{proof}
    See Appendix~\ref{proof_prop_derivative_loss_Fh}
\end{proof}

%%---------- End of Proposition ------------






%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%% SUB - SECTION %%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsubsection{Steepest descent formulation} 
%
By leveraging the results in Proposition~\ref{prop_derivative_loss_Fh} we propose a steepest descend algorithm to compute the value of the filters $\boldsymbol{h}$ that minimize the cost function 
%
%
$
\ell(
    \boldsymbol{h}
    )
    =\frac{1}{2}
         \left\Vert 
               \boldsymbol{r}
               -
               F\left(
                    \boldsymbol{h}
                \right)    
         \right\Vert_{\calH(K)}^2
.
$
%
%
To show this we start recalling that given $\ell(\boldsymbol{h})$ and its Fr\'echet derivative we have 
%
%
%
\begin{equation}
\ell\left( 
        \boldsymbol{h}_{k}
        +
        \alpha
        \boldsymbol{d}
    \right)
=
\ell(\boldsymbol{h}_{k})
+
\bbD_{\ell}(\boldsymbol{h}_{k})
   \left\lbrace 
        \alpha\boldsymbol{d}
   \right\rbrace
+
o\left( 
     \boldsymbol{h}
 \right)
 ,
\end{equation}
%
%
%
which in the light of Proposition~\ref{prop_derivative_loss_Fh} leads to
%
%
%
\begin{multline}
\ell\left( 
        \boldsymbol{h}_{k}
        +
        \alpha
        \boldsymbol{d}
    \right)
=
\\
\ell(\boldsymbol{h}_{k})
     -
     \alpha
     \left\langle 
           \bbD_{F}(\boldsymbol{h}_{k})\left\lbrace 
                                        \boldsymbol{d} 
                                   \right\rbrace
           ,  
           \boldsymbol{r}
           -
           F(\boldsymbol{h}_{k})
    \right\rangle_{\ccalH(K)}
+
o\left( 
     \boldsymbol{h}
 \right)
 .
\end{multline}
%
%
%
Then, to find the direction, $\boldsymbol{d}$, of the fastest decrease we must select $\boldsymbol{d}$ as the solution to the following problem.
%
%
%
\begin{equation}
   \sup_{\boldsymbol{d}}
       \left\langle 
           \bbD_{F}(\boldsymbol{h}_{k})\left\lbrace 
                                        \boldsymbol{d} 
                                   \right\rbrace
           ,  
           \boldsymbol{r}
           -
           F(\boldsymbol{h}_{k})
    \right\rangle_{\ccalH(K)}
    ~
    \text{s.t.}
    ~
    \Vert \boldsymbol{d}\Vert_{\ccalH(K)}=1
    .
\end{equation}
%
%
%
The solution of this problem is achieved when $\boldsymbol{d}$ is selected such that
%
%
%
\begin{equation}\label{eq_inner_prod_eqmax}
 \bbD_{F}(\boldsymbol{h}_{k})
     \left\lbrace 
          \boldsymbol{d}
     \right\rbrace
     =
      \boldsymbol{r}
      -
      F(\boldsymbol{h}_{k})
      .
\end{equation}
%
%
%
If we denote the solution of~\eqref{eq_inner_prod_eqmax} by $\tilde{\boldsymbol{d}}_{k}$, then we have that the values of $\boldsymbol{h}$ in the $k$-step of an iterative search is given by
%
%
%
\begin{equation}\label{eq_iter_hk}
\boldsymbol{h}_{k+1}
=
\boldsymbol{h}_{k}
+
\alpha_{k} 
\boldsymbol{d}_{k}
,
\end{equation}
%
%
%
where 
%
%
$
\boldsymbol{d}_{k} = \tilde{\boldsymbol{d}}_{k} / \Vert \tilde{\boldsymbol{d}}_{k} \Vert_{\ccalH(K)}
,
$
%
%
and where the values of $\alpha_{k}$ can be selected according to the so called Wolfe conditions~\cite{nocedal2006numerical}.

In what follows we make explicit, in Algorithm~\ref{alg_get_d} and Algorithm~\ref{alg_alphak_update_rule}, how to solve~\eqref{eq_inner_prod_eqmax} using a conjugate gradient descent and how to select the values of $\alpha_{k}$ in~\eqref{eq_iter_hk}.





%%------------------------------------------
%%-------------- ALGORITHM -----------------
%%------------------------------------------

\begin{algorithm}
%
%
\caption{
Finding $\boldsymbol{d}$ in
$
\bbD_{F}(\boldsymbol{h})
     \left\lbrace 
          \boldsymbol{d}
     \right\rbrace
=
    \boldsymbol{r}
    -
    F(\boldsymbol{h})
    .
$      
}\label{alg_get_d}
%
%
\begin{algorithmic}
\Require $\boldsymbol{h}$, $F(\boldsymbol{h})$, $\boldsymbol{r}$, $\bbD_{F}(\boldsymbol{h})\{ \cdot \}$
\Ensure $\boldsymbol{d}$
%
%
\State $\boldsymbol{d}_{0} = 0$
%
\State $\boldsymbol{s}_{0} = \boldsymbol{r}
    -
    F(\boldsymbol{h})
    -
    \bbD_{F}(\boldsymbol{h})
     \left\lbrace 
          \boldsymbol{d}_{0}
     \right\rbrace
    $
%
%
\State $\boldsymbol{p}_{0} = \boldsymbol{s}_{0}$
%
\State $k=0$
%
\State $\texttt{aux}=1$
%
\While{$\texttt{aux}=1$}
\State 
%
$\displaystyle
\gamma_{k}
   =
   \frac{
        \left\langle 
               \boldsymbol{s}_{k}
               ,
               \boldsymbol{s}_{k}
        \right\rangle_{\ccalH(K)}
        }
        {
        \left\langle 
               \boldsymbol{p}_{k}
               ,
               \bbD_{F}(\boldsymbol{h})\{ \boldsymbol{p}_{k} \}
        \right\rangle_{\ccalH(K)}
        }
$
%
\State $\boldsymbol{d}_{k+1} = \boldsymbol{d}_{k} + \gamma_{k}\boldsymbol{p}_{k
}$
%
\State $\boldsymbol{s}_{k+1} = \boldsymbol{s}_{k} - \gamma_{k}\bbD_{F}(\boldsymbol{h})\{ \boldsymbol{p}_{k} \}$
%
%
\If{$\Vert \boldsymbol{s}_{k+1}\Vert_{\ccalH(K)}<\epsilon$}  
    \State $\boldsymbol{d}=\boldsymbol{d}_{k+1}$ 
    \State $\texttt{aux}=0$
\Else
    \State 
%
$\displaystyle
\beta_{k}
   =
   \frac{
        \left\langle 
               \boldsymbol{s}_{k+1}
               ,
               \boldsymbol{s}_{k+1}
        \right\rangle_{\ccalH(K)}
        }
        {
        \left\langle 
               \boldsymbol{s}_{k}
               ,
               \boldsymbol{s}_{k}
        \right\rangle_{\ccalH(K)}
        }
$
%
\State $\boldsymbol{p}_{k+1}=\boldsymbol{s}_{k+1}+\beta_{k}\boldsymbol{p}_{k}$
%
\State $k=k+1$
%
\EndIf
\EndWhile
%
\end{algorithmic}
\end{algorithm}

%%------------ End of Algorithm ------------








%%------------------------------------------
%%-------------- ALGORITHM -----------------
%%------------------------------------------

\begin{algorithm}
\caption{Update rule for $\alpha_k$ in~\eqref{eq_iter_hk}}\label{alg_alphak_update_rule}
%
%
\begin{algorithmic}
\Require $\overline{\alpha}>0$, $\rho\in (0,1)$, $c\in (0,1)$
\Ensure $\alpha_k$
%
\State $\alpha = \overline{\alpha}$
%
\State $\texttt{aux}=1$
%
\While{$\texttt{aux}=1$}
\If{
\begin{equation*}
\boldsymbol{\ell}\left(
                    \boldsymbol{h}_{k}
                    +
                    \alpha
                    \boldsymbol{d}_{k}
                 \right) 
                 \leq 
\boldsymbol{\ell}\left(
                     \boldsymbol{h}_{k}
                 \right) 
                 -
                 c
                 \alpha
                 \left\langle 
           \bbD_{F}(\boldsymbol{h}_{k})\left\lbrace 
                                        \boldsymbol{d}_{k} 
                                   \right\rbrace
           ,  
           \boldsymbol{r}
           -
           F(\boldsymbol{h}_{k})
    \right\rangle_{\ccalH(K)}
\end{equation*}
}
\State $\texttt{aux}=0$
%
\Else
   \State $\alpha \gets \rho \alpha$
\EndIf   
\EndWhile
\State $\alpha_{k}= \alpha$
\end{algorithmic}
\end{algorithm}

%%------------ End of Algorithm ------------






==> v12/sec_spectral_representations_algrkhs.tex <==
%!TEX root =../compiler_paper.tex





%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%% SECTION %%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\section{Spectral Representations}

\alejandropm{HERE I WILL RECHECK IF THIS DISCUSSION IS ACTUALLY NECESSARY}












